One Size Fits All for Semantic Shifts: Adaptive Prompt Tuning for Continual Learning

In real-world continual learning (CL) scenarios, tasks often exhibit intricate and unpredictable semantic shifts, posing challenges for fixed prompt management strategies which are tailored to only handle semantic shifts of uniform degree (i.e., uniformly mild or uniformly abrupt). To address this limitation, we propose an adaptive prompting approach that effectively accommodates semantic shifts of varying degree where mild and abrupt shifts are mixed. AdaPromptCL employs the assign-and-refine semantic grouping mechanism that dynamically manages prompt groups in accordance with the semantic similarity between tasks, enhancing the quality of grouping through continuous refinement. Our experiment results demonstrate that AdaPromptCL outperforms existing prompting methods by up to 21.3%, especially in the benchmark datasets with diverse semantic shifts between tasks.

==> backup_3-Methodology.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

% \noindent\textbf{Continual Learning.}
\subsection{Continual Learning}
%In continual learning, we encounter a sequence of tasks $D = \{D_1, \dots, D_T\}$, with $T$ denoting the total number of encountering tasks. Task $t$ has a data stream $D_t = \{(x^i_t, y^i_t)\}_{i=1}^{m_t}$ derived from a joint distribution over input space $\mathcal{X}_t$ and one-hot encoded label space $\mathcal{Y}t$, with $m_t$ being the number of instances for that task. The goal in continual learning is to formulate a classifier that maximizes test accuracy for all encountered tasks $\{1, 2, \dots, T\}$, with restricted access to the data streams $D_{t^{\prime}}$ of prior tasks where $t^\prime < t$. In realistic CL scenarios, these data streams may exhibit diverse environments and varying inter-task similarities, serving as a comprehensive testbed for evaluating the adaptability of continual learning approaches.

In CL, we consider a sequence of tasks $t$ for a data stream $D = \{D_1, \dots, D_T\}$, where each sub-data stream $D_t = \{(x^i_t, y^i_t)\}_{i=1}^{m_t}$ for a task $t$ with $m_t$ data instances is derived from a joint distribution of an input space $\mathcal{X}_t$ and a label space $\mathcal{Y}_t$. The primary goal in CL is to continuously learn a classifier over $D$ that maximizes test accuracy for all encountered tasks $\{1, 2, \dots, t\}$ up to $t$, without having access to the data streams $D_{t^{\prime}<t}$ of prior tasks. In realistic settings, these data streams may originate from diverse environments and thus associated tasks exhibit varying inter-task similarities, calling for adaptable CL approaches.


\smallskip
% \noindent\textbf{Prompt Tuning Continual Learning.}
\subsection{Prompt Tuning Continual Learning}
%Current prompt-based continual learning methods\,\cite{l2p, dp, lae} mostly employ a pretrained backbones like ViT, which is primarily composed of $L$ transformer blocks. Each of these blocks utilizes a multi-head attention module to extract pertinent features. Then, prompts, small additional weight parameters, are prepended as additional input for the transformer block's attention module. Recently, as discussed in \cite{DP, LAE}, prompts primarily serve as a prefix, prepending exclusively to the keys and values of the input. A single prompt ${\rm P} \in \mathbb{R}^{p \times d}$ is defined as a sequence of tokens, each with $d$ dimensions, and the sequence has a length of $p$. This prompt is compatible with key and value configurations in various prompt-based CL techniques. 
%
%
% In the context of our study, let ${\rm {E}}_l \in \mathbb{R}^{n \times d}$ denote the input tokens, introduced to the $l$-th transformer block. Then, the attention mechanism can then be reformulated as:
% \begin{equation}
% \begin{gathered}
% {\rm {E}}^\prime_{l} = {\rm Attention}({\rm {Q}}, {\rm {K^\prime}}, {\rm {V^\prime}}) ~\text{where}~ \\
% {\rm {Q}} = {\rm {E}}_l{\rm W}^Q,~{\rm {K^\prime}} = [{\rm P}; {\rm {E}}_l{\rm W}^K],~{\rm {V^\prime}} = [{\rm P}; {\rm {E}}_l{\rm W}^V].
% \end{gathered}
% \label{eq:attn_prompts}
% \end{equation}
% Here, ${\rm W}^Q$, ${\rm W}^K$, and ${\rm W}^V$ denote the linear projection matrices for the query, key, and value input tokens, in that order. The symbol $[\cdot;\cdot]$ represents concatenation, and a single-head attention mechanism is defined as
% % ${\rm W}^Q$, ${\rm W}^K$, and ${\rm W}^V$ are linear projections matrices for query, key, and value tokens, respectively; $[\cdot;\cdot]$ is concatenation; and the attention mechanism is defined as: 
% \begin{equation}
% {\rm Attention}({\rm {Q}}, {\rm {K}}, {\rm {V}})=\rm{softmax}\left(\frac{{\rm Q}{\rm K}^T}{\sqrt{d}}\right){\rm V}
% \label{eq:attn}
% \end{equation}
%
Recent prompt-based CL methods\,\cite{l2p, dp, lae} mostly employ a pretrained backbone (e.g., ViT\,\cite{}) with $L$ transformer blocks, where each of these blocks utilizes a multi-head attention module to extract pertinent features. A prompt, in this context, refers to a set of vectors that provide context or guide the attention mechanism towards specific patterns in the data, defined as:
\begin{equation}
{\rm P} = [{\rm \mathbf{p}}_1,\dots, {\rm \mathbf{p}}_p ] \in \mathbb{R}^{p \times d}
\label{eq:prompt}
\end{equation}
where $p$ represents the number of prompt tokens ${\rm \textbf{p}}_i$ while $d$ denotes the dimensionality of each prompt. These prompts serve as a prefix input for the transformer block's attention module, prepended exclusively to the keys and values\,\cite{DP, LAE}.
Specifically, given input tokens ${\rm {E}}_l \in \mathbb{R}^{n \times d}$ at an $l$-th transformer block, a prompt ${\rm P}$ is incorporated as follows to produce output tokens ${\rm {E}}^\prime_{l}$:
\begin{equation}
\begin{gathered}
{\rm {E}}^\prime_{l} = {\rm Attention}({\rm {Q}}, {\rm {K^\prime}}, {\rm {V^\prime}}) ~\text{where}~ \\
{\rm {Q}} = {\rm {E}}_l{\rm W}^Q,~{\rm {K^\prime}} = [{\rm P}; {\rm {E}}_l{\rm W}^K],~{\rm {V^\prime}} = [{\rm P}; {\rm {E}}_l{\rm W}^V],
\end{gathered}
\label{eq:attn_prompts}
\end{equation}
where ${\rm W}^Q$, ${\rm W}^K$, and ${\rm W}^V$ respectively denote the linear projection matrices for the input tokens to query $Q$, key $K$, and value $V$. Here, $[\cdot;\cdot]$ represents concatenation, and a single-head attention is defined as
\begin{equation}
{\rm Attention}({\rm {Q}}, {\rm {K}}, {\rm {V}})=\rm{softmax}\left(\frac{{\rm Q}{\rm K}^T}{\sqrt{d}}\right){\rm V}.
\label{eq:attn}
\end{equation}
%
%In this framework, while the pre-trained backbone remains fixed, the prompts are the main elements subjected to learning. Consequently, these prompts influence the output embeddings of the ViT’s transformer layers by permeating to the image patch tokens through attention mechanisms, thereby adapting to the specific task at hand.
%
While the pre-trained backbone remains unchanged, the prepended prompts are optimized while attending to the input tokens, thereby adapting to specific tasks at hand.

%%%%

\section{Proposed Method: \algname{}}
\label{sec:methodology}
% \algname{} realizes adaptive prompt management for tasks with diverse semantics through semantic-aware adaptation. The strategy focuses on maximizing the positive transfer between CL tasks by universally learning tasks with relevant semantics while specifically targeting tasks that present novel semantics. Following this, tasks are learned using prompts that correspond to the carefully determined semantics. Finding the optimal task grouping is infea
% To achieve both precision in task grouping and computational efficiency

% \textit{semantic-based hierarchical task grouping} based on (a) \textit{macroscopic semantic assignment} and (b) \textit{microscopic semantic refinement}. To achieve both precision in task grouping and computational efficiency, the former phase allocates tasks by performing a broad-level semantic assignment, while the latter phase focuses on precisely refining assignments by additionally taking into account the semantics of more relevant tasks.
% The overall procedure is depicted in Figure \ref{fig:model_arch} and outlined in Algorithm \ref{alg:overall}.

% The strategy centers around universally learning tasks with relevant semantics while specifically targeting tasks that present novel semantics. Following this, tasks are learned using prompts that correspond to the carefully determined semantics. 

% Given the unpredictability of future tasks, this refinement is designed to occur any time the semantics of previous and new tasks become universal in the future. 

% \input{figures/algorithm}
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.98\textwidth, ]{figures/model_arch.pdf}
    % \includegraphics[width=0.95\textwidth, ]{figures/model_arch.pdf}
    \caption{\textbf{Detailed view of the main components of \algname{}}:
    }
    \label{fig:model_arch}
    % \vspace*{-0.6cm}
\end{figure*}

\subsection{Overview: Hierarchical Semantic Grouping}
\label{subsec:prompt-assigning}
% aim
% addressing diverse tasks in CL by universally learning tasks with relevant semantics; and non-universally targeting tasks with novel semantics.
% Our primary objective is to address the challenge of learning from diverse tasks in CL. The strategy centers around universally learning tasks with relevant semantics while specifically targeting tasks that present novel semantics.
\algname{} realizes adaptive prompt management for CL tasks through \textit{semantic}-aware adaptation. The key strategy is to universally learn tasks with relevant semantics while specifically targeting tasks that present novel semantics. Following this, tasks are learned using prompts that correspond to the carefully determined semantics. The overall procedure is depicted in Figure \ref{fig:model_arch} and outlined in Algorithm \ref{alg:overall}.


% \textit{semantic-based hierarchical task grouping} based on (a) \textit{macroscopic semantic assignment} and (b) \textit{microscopic semantic refinement}. To achieve both precision in task grouping and computational efficiency, the former phase allocates tasks by performing a broad-level semantic assignment, while the latter phase focuses on precisely refining assignments by additionally taking into account the semantics of more relevant tasks.
% The overall procedure is depicted in Figure \ref{fig:model_arch} and outlined in Algorithm \ref{alg:overall}.

Central to \algname{} is the concept of \textit{semantics}, which pertains to the intrinsic patterns insights tied to a task's data distribution. For instance, Figure \ref{fig:model_arch}(a) indicates that Task 3 and 4 classify images within the realms of architectural and satellite semantics, respectively. To capture this, we define the notion of a \textit{task semantic embedding}---a vector representation that encapsulates the core essence of a task---in Definition \ref{def:task_semantic_embedding}. This vector is derived using a prompt from Eq.~\eqref{eq:prompt} over a warm-up training period. 
\begin{definition}{\sc (Task Semantic Embedding)}.
Given warm-up prompt \( {\rm P}^w_t \) for task \( t \), the \textit{task semantic embedding} is computed as
\begin{equation}
e_t = {\rm Normalize}\left({\rm AvgPool}({\rm P}^w_t)\right) \in \mathbb{R}^{d},
\label{eq:task_semantic_embedding}
\end{equation}
where {\rm AvgPool($\cdot$)} is a function that aggregates the outputs across all $p$ lengths, encapsulating the semantics for task $t$ and {\rm Normalize($\cdot$)} performs $l_2$-normalization.
\label{def:task_semantic_embedding}
\end{definition}

Building on this, the objective of \algname{} is to find the particular partitioning\,(clustering) of CL tasks into semantic groups that maximize the total intra-cluster similarity, leading to the maximal positive transfer. Such a cluster is termed a \textit{semantic group}, outlined as: 
\begin{definition}{\sc (Semantic Group)}.
The \textit{semantic group} for a semantic $s$ is represented as 
\begin{equation}
G_s = \{ t~ |~ \psi(t)=s, ~ t\in \{1,\dots,T\}\},
\label{eq:task_semantic_group}
\end{equation}
where $\psi(t)$ returns an assigned semantic for a given task $t$.
\label{def:task_semantic_group}
\end{definition}
\noindent 
% This semantic group can be as few as one when all tasks share similar semantics or as many as $t$ for completely distinct tasks. 
Formally, we aim to find optimal semantic grouping $G^*$ such that
\begin{equation}
G^* = \underset{{G}}{\mathrm{argmax}} \left( \sum_{i=1}^{|G|} \sum_{t_1, t_2 \in G_i} {\rm Similarity}(e_{t_1}, e_{t_2}) \right)
\label{eq:obj}
\end{equation}
where ${G}$ is the set of semantic groups defined as ${G}=\{ G_1, \dots, G_{|G|} \}$, and ${\rm Similarity}(e_{t_1}, e_{t_2})$ denotes the similarity between task semantic embeddings $e_{t_1}$ and $ e_{t_2}$. 

% Furthermore, in CL, the diverse and sequential nature of tasks often gives rise to order sensitivity.
Solving this optimization problem directly is computationally infeasible due to its combinatorial nature and the inherent inaccessibility of CL to previous or upcoming tasks.
Furthermore, in CL, as tasks are processed sequentially without a global view of entire tasks, such a short-sighted, or greedy, assignment approach often causes incorrect semantic grouping. Though reassignment of processed tasks can rectify these errors, it is computationally inefficient if applied indiscriminately.

To achieve both precision in semantic grouping and computational efficiency, \algname{} introduces a \textit{two-level hierarchical semantic grouping}, drawing inspiration from the pre-clustering algorithm\,\cite{canopy}. Initially, we aim to identify \textit{macroscopic semantic groups} that grasp global semantics of CL tasks\,(Section \ref{subsec:mac}). Subsequently, we refine these groups to determine the final \textit{semantic groups} as per Definition \ref{def:task_semantic_group}\,(Section \ref{subsec:mic}). 

Finally, these semantic groups form the basic elements for training prompts and subsequent inferences\,(Section \ref{subsec:tr_inf}). As tasks undergo refinement from non-universal to universal, there arises a potential mismatch where prompts aligned with these tasks may remain unprocessed. To maintain the adaptability of the refinement, we identify candidate sub-semantic groups that, while currently designated as non-universal, show strong potential for merging in the future. \algname{} proactively pre-tunes and reserves prompts for these candidate groups.

\input{figures/algorithm}

% In addition, as tasks transition during the refinement\,(the latter phase) from being categorized as non-universal to universal, we often encounter scenarios where the prompts trained on these tasks have not been processed. Thus, to maintain the adaptability of the refinement, we identify candidate sub-semantic groups that, while currently designated as non-universal, show strong potential for merging in the future. For these candidate groups, \algname{} proactively pre-tunes and reserves prompts for future use.

% Basic concepts: Definitions of Semantic, Semantic group
% Central to \algname{} is the idea of semantics, which represents the inherent meaning or set of meanings within a task. To quantify this, we define a task's "semantic embedding," a vector representation capturing its essence using a prompt in Eq. (?) tuned to task data. + def. of task semantic embedding
% The overall strategy of \algname{} is to group tasks with similar semantics, forming what we refer to as a "semantic group". + def. of semantic group

% why two-level?
% CL often suffers from order sensitivity\,\cite{kmeans, etc.} since the assignment of tasks is done sequentially without a global view of all tasks, a greedy approach can misclassify tasks into wrong semantic groups.
2e% For precise assignment, Reassignments of tasks can be effective but computationally inefficient if applied indiscriminately.

% To counteract this: \algname performs two-level hierarchical task assignment. 
% This assignment approach is reminiscent of the pre-clustering algorithm\,\cite{canopy} that ensures both computational efficiency and precision in task groupings. Our goal is to first identify \textit{macroscopic semantic groups} and subsequently concentrate refinement efforts on each macroscopic group to segment into \textit{microscopic sub-semantic groups} that properly align tasks with their true semantic categories

% Prompt tuning and inference
% Then, sub-semantic groups are the units of training prompts and inference.
% Thus, \algname{} independently learns a prompt for each sub-semantic group to capture the information shared among corresponding tasks
% However, in the refinement process in Eq.~\eqref{eq:micro_refine} where tasks transitioning from a previously non-universal to a universal status necessitate the prompts trained on these tasks already processed, we may lack such prompts. 
% For the versatility of \algname{} in rehearsal-free CL, \algname{} identifies candidate sub-semantic groups, currently designated as non-universal but demonstrating strong potential for merging in the future and pre-tunes and reserves prompts for these candidate groups.


% In addressing diverse task semantics in CL, we universally learn semantically similar tasks, while specifically targeting tasks that are dissimilar. To achieve this, we compare the semantics of a task with existing ones and assign the tasks for tuning either universally or specifically.
% However, the sequential nature of semantic assignments in CL, lacking a global view of all tasks can make the quality of assignments susceptible to task order, as aligned with findings in online clustering literature\,\cite{kmeans, etc.}. This often leads to over-grouping where the number of identified semantic groups exceeds the ideal as illustrated in Figure \ref{fig:order-sensitivity}. To mitigate this, \algname{} strategically employs macro-level semantic groupings to allow refinements in subsequent phases.

\subsection{Phase 1: Macroscopic Semantic Assignment}
\label{subsec:mac}
Initially, \algname{} captures global semantics in the CL distribution via \textit{macroscopic semantic groups}, in Definition \ref{def:macro_semantic_group}. Simultaneously, these semantic groups allow opportunities for future refinements for the final semantic grouping.

\begin{definition}{\sc (Macroscopic Semantic Group)}
Let $\tau_1$ denote the distance threshold indicating highly divergent semantic difference. The \textit{macroscopic semantic group} for a macro-level semantic $m$ comprises a collection of tasks that maintain an internal distance smaller than the threshold, $\tau_1$. That is,
\begin{equation}
\mathcal{G}_m = \{t~|~ {\rm Avg\text{-}Dist}(\mathcal{G}_m) \leq \tau_1 \},
\label{eq:macro_semantic_group}
\end{equation}
where \({\rm Avg\text{-}Dist}(\mathcal{G}_m)\) computes the internal distance to its centroid as $\left( \frac{1}{|\mathcal{G}_m|} \sum_{t \in \mathcal{G}_m} \left( e_t - {\rm Centroid}(\mathcal{G}_m) \right)^2 \right)^{1/2}$ and ${\rm Centroid}(\mathcal{G}_m) = \frac{1}{|\mathcal{G}_m|}\sum_{t \in \mathcal{G}_m} e_t$.

\label{def:macro_semantic_group}
\end{definition}

Upon the arrival of a new task, as illustrated in Figure \ref{fig:model_arch}(a), \algname{} performs a \textit{sequential clustering} with $\tau_1$, \(\rm Seq{\text -}cluster_{\tau_1}(\cdot)\). This involves estimating the \textit{semantic distance} between the new task and the existing macroscopic semantic groups, followed by assigning the new task to the most appropriate group. 

\smallskip
\noindent\textbf{Semantic Distance Estimation.} 
\textit{Semantic distance} of a new task against existing semantic groups is measured as the internal distance within a new task's semantic embedding and those of the closest semantic group, as formulated in Definition \ref{def:task_semantic_distance}.
\begin{definition}{\sc (Semantic Distance)}.
Given the semantic group features \(\{\mathcal{G}_1, \ldots, \mathcal{G}_{|{\mathcal{G}}|} \}\), and a new task \(t\), the \textit{semantic distance} is
\begin{equation}
\begin{gathered}
d_t = {\rm Avg\text{-}Dist}\left(\mathcal{G}_{m^*} \cup \{t\}\right), \\
\text{~where~} m^* = \arg\min_{m} {\rm d}\left( {\rm Centroid}\left(\mathcal{G}_m\right), e_t \right),\\
\end{gathered}
\label{eq:task_semantic_distance}
\end{equation}
and \({\rm d}(\cdot,\cdot)\) denotes the Euclidean distance between two vectors.
\label{def:task_semantic_distance}
\end{definition}

\noindent\textbf{Macroscopic Assignment.} 
As a result of the macroscopic assignment, (i) a task with a large distance\,($d_t > \tau_1$) is directed to a newly-initialized macroscopic semantic group due to its \textit{novel semantic}; (ii) a task with relevant semantic distance\,($d_t \leq \tau_1$) is allocated to an existing macroscopic semantic group due to its \textit{relevant semantic}.
For a task with semantic distance $d_t$, its assignment to a macroscopic semantic group is represented as:
\begin{equation}
% \mathcal{G}(t) \leftarrow{}
\begin{cases}
\mathcal{G}_{|\mathcal{G}|+1} = \{t\} & \text{if } d_t > \tau_1 \quad \text{(i) Novel Semantic,} \\
\mathcal{G}_{m^*} \cup \{t\} & \text{if } d_t \leq \tau_1 \quad \text{(ii) Relevant Semantic.}
\end{cases}
\label{eq:mac_assign}
\end{equation}
The closest semantic index $m^*$ is derived from Eq.~\eqref{eq:task_semantic_distance}. 
% Here, $\mathcal{G}(t)$ denotes the macroscopic semantic group allocated to task $t$. 

% Refining these semantic groups can be effective but computationally expensive if applied indiscriminately. Thus, we propose an assignment approach reminiscent of the pre-clustering algorithm\,\cite{canopy} where our goal is to first identify \textit{macroscopic semantic groups} and subsequently concentrate refinement efforts on tasks with marginal differences, ensuring both computational efficiency and precision in task groupings.
% Specifically, as a result of the assignment, (i) a task with clearly large distance is directed to a newly-initialized semantic group to \textit{specifically} tune on a novel task; (ii) a task with neutral semantic distance is allocated to an existing semantic group, which is \textit{remergable} by further refinement.

% The overall task assignment is controlled by two distance thresholds, $\tau_1$ and $\tau_2$, with $\tau_1 > \tau_2$. 
% While $\tau_1$ acts as a preliminary mechanism for clustering tasks with significantly distinct semantics, $\tau_2$ ultimately determines if a task aligns universally or specifically with existing semantics.
% Thus, for a task with semantic distance $d_t$, the macroscopic semantic group is determined by $\tau_1$,
% \begin{equation}
% G(t) \leftarrow{}
% \begin{cases}
% G_{|G|+1} = \{e_t\} & \text{if } d_t > \tau_1 \quad (\text{Specific}) \\
% G_{s^*} \cup \{e_t\} & \text{if } d_t \leq \tau_1 \quad (\text{Remergable})
% \end{cases}
% \end{equation}
% Here, $G(t)$  denotes the macroscopic semantic group allocated to task $t$. The closest semantic index $s^*$ is derived from Eq.~\eqref{eq:task_semantic_distance}. 

\subsection{Phase 2: Microscopic Semantic Refinement}  
\label{subsec:mic}
In microscopic refinement, we determine the final semantic grouping as per Definition \ref{def:task_semantic_group} while focusing on the precise partitioning of macroscopic semantic groups.
Here, we segment a macroscopic semantic group into the final \textit{semantic groups} by employing a more granulated threshold $\tau_2$ where $\tau_1 > \tau_2$, represented as:
\begin{equation}
S(\mathcal{G}_m) = \{ G^1_m, \dots, G^{r_m}_m \} \text{~~where~~} \mathcal{G}_m = \bigcup_{i=1}^{r_m} G^i_m,
\label{eq:micro_refine}
\end{equation}
$G^i_m$ indicates the $i$-th semantic group for the macroscopic semantic group $\mathcal{G}_m$. The $r_m$ indicates the least number of semantic groups ensuring the internal distance within each is limited to $\tau_2$, i.e., $ {\rm Avg\text{-}Dist}(G^i_m) \leq \tau_2$. If the macroscopic semantic group's radius already satisfies the condition, i.e., \({\rm Avg\text{-}Dist}(G_s) \leq \tau_2\), the refinement is skipped and the semantic group maintains the identity of $\mathcal{G}_m$.

The main idea of refinement is to avoid task order sensitivity inherent to the sequential semantic assignments in CL. Thus, we present a simulation-based refinement strategy that utilizes simulations to execute assignments over varied virtual task orders. As an illustration in Figure \ref{fig:model_arch}(b), consider a scenario where the two semantic groups generated by an original task order can be refined into a single group informed by an alternative task order. 
In detail, starting with the original task order within a macroscopic semantic group $\mathcal{G}_m$, virtual task orders are generated through permutation as \(\Bar{\mathcal{G}}_m = {\rm Perm}(\mathcal{G}_m)\). We then perform the sequential clusterings with \(\tau_2\) on the generated task orders, \(\rm Seq{\text -}cluster_{\tau_2}(\cdot)\), to identify the task order $\Bar{\mathcal{G}}^*_m$ that yields the fewest semantic groups as:
\begin{equation}
\Bar{\mathcal{G}}^*_m = \arg\min_{\Bar{G}_{s}} \rm{Count}({\rm Seq{\text -}cluster}_{\tau_2}(\Bar{\mathcal{G}}_m)),
\end{equation}
where ${\rm Count}(\cdot)$ quantifies the semantic groups generated for a specific task order.
Lastly, we obtain the final semantic groups, in Eq.~\eqref{eq:micro_refine}, of a macroscopic semantic through ${\rm Seq{\text -}cluster}_{\tau_2}(\Bar{\mathcal{G}}^*_m)$. 

% In the refinement process in Eq.~\eqref{eq:micro_refine}, tasks transitioning from a previously non-universal to a merged status necessitate the prompts trained on these tasks already processed. The challenge arises as we may lack such prompts adapted to these passed tasks and assessing such tasks' data is non-permissible. Given the constraints of a rehearsal-free CL, \algname{} emphasizes the necessity to pre-tune prompts for these tasks.
% \algname{} emphasizes the necessity to pre-tune prompts for these tasks.

% $\arg\max_{c} {\rm Silhouette}({\rm K\text{-}Means}(G_s, c))$.
% As elaborated in Section x.x, this method manifests a decline in performance.

% While we train a prompt and a key for each microscopic sub-semantic group, for the use of the dynamic refinement process in Eq.~\eqref{eq:micro_refine} in rehearsal-free CL, \algname{} also pre-tune these for sub-semantic groups with strong potential for future refinements. First, \algname{} identifies sub-semantic groups currently designated as non-universal but demonstrate strong potential for merging in the future. Without relying on the distance threshold, we select multiple candidate sets of sub-semantic groups, $C(G_s)$, by employing a clustering method with the number of clusters informed by a distributional indicator. Formally, a single candidate set is represented as:

% to maintain the adaptability of the refinement process in Eq.~\eqref{eq:micro_refine}, our optimization involves preparation for potential refinement where 
% pre-tuning prompts and keys based on their potential for future refinements.

\subsection{Training and Inference}  
\label{subsec:tr_inf}
The carefully determined semantic groups serve as basic elements for both prompt tuning and inference. Each of these groups has a prompt and associated key, symbolized as $({\rm P}^i_j, {\rm k}^i_j)$ for a group $G^i_j$.
In addition, to prepare tasks transition from being categorized as non-universal to universal by the refinement in Eq.~\eqref{eq:micro_refine}, \algname{} proactively tunes prompts for candidate semantic groups with strong potential for merging.

\smallskip
\noindent\textbf{Potential Refinement Preparation.}
\algname{} first identifies candidate sub-semantic groups currently designated as non-universal but demonstrate strong potential for merging in the future.
Thus, without relying on the distance threshold, multiple candidate sets of semantic groups, $C(\mathcal{G}_m)$, are selected through multiple runs of clustering, where the cluster count is pre-determined by a distribution indicator, e.g., silhouette score\,\cite{silhouette}. Formally, a single candidate set is obtained by:
\begin{equation}
C^{i}(\mathcal{G}_m) = {\rm K\text{-}means}_{c^*}(\mathcal{G}_m),
\label{eq:candidate_sets}
\end{equation}
where $c^*$ is the determined cluster number by the silhouette score.
We also investigate the consequences of post-merging without adaptation to prior tasks, such as by averaging the prompts' parameters in Section \ref{subsec:anal_micro_refine}.

\smallskip
\noindent\textbf{Overall Optimization.}
% denoted as (P^i_j,k^i_j),
We optimize the prompts and the associated keys for the semantic groups, obtained in Eq.~\eqref{eq:micro_refine} and \eqref{eq:candidate_sets}, that encompass the current task $t$, formulated as: 
\begin{equation}
\small
    \theta_t = \{ ({\rm P}^i_j, {\rm k}^i_j)~ |~t \in G^i_j \text{~~and~~} G^i_j \in S(\mathcal{G}_m) \cup C(\mathcal{G}_m) \}.
\label{eq:prompts4tuning}
\end{equation}
% To obtain generalizability across a semantic group $G^i_j$, 
We initialize the parameters of a semantic group $G^i_j$ with the pre-tuned those of the group $G^i_j\setminus\{t\}$ and fine-tune them on the current task. For tasks introducing a novel semantic, the parameters are trained from scratch. Overall, the optimization objective for each task $t$ is formulated as:
\begin{equation}
\small
\min_{({\rm P}, {\rm k})\in\theta_t, \phi} \ell_{ce} (f_\phi(f_{\rm P}(x_t)[\mathtt{CLS}]), y_t) - \lambda{\rm Cosine}(q(x_t),{\rm k}), 
\label{eq:objective}
\end{equation}
where $f_{\rm P}$ transforms the input tokens using prompts as Eq.~\eqref{eq:attn_prompts}, and then forwards them to the pre-trained backbone, and $f_\phi$ is the classifier utilizing the [$\mathtt{CLS}$] token for prediction; $\rm{Cosine}(\cdot)$ denotes the cosine similarity function and $q(x)$ is the feature vector of the [$\mathtt{CLS}$] token from the pre-trained backbone. $\ell_{ce}$ and $\lambda$ denote the cross-entropy loss and a balancing coefficient between two loss terms, respectively.


\smallskip
\noindent\textbf{Semantic Group Inference.}
Inference of the semantic group identity is necessary for application purposes. As the task identity prediction mechanism in \cite{l2p, dp}, each microscopic semantic group $G^i_j$ is inferred through the matching of the keys, which are optimized by Eq.~\eqref{eq:objective}. Given a test instance $x$, its semantic group identity is determined by:
\begin{equation}
\hat{i}, \hat{j} = \arg\max_{i,j} {\rm Cosine}(q(x), {\rm k}^i_j).
\label{eq:inference}
\end{equation}
% where $\rm{Cosine}(\cdot)$ denotes the cosine similarity function and $q(x)$ represents the feature vector tied to the [$\mathtt{CLS}$] token from our pre-trained architecture.


% for intermediate tasks
% This can make the quality of assignments susceptible to task order, especially with tasks having intermediate distances, leading to over-grouping where the number of identified semantic groups exceeds the ideal as described in Figure \ref{fig:order-sensitivity}. Such order-dependency, a known challenge in traditional clustering algorithms,\cite{kmeans, etc.}, is even more pronounced in online clustering. 
% Although tasks with clearly large or small distances provide groupings consistent with global clustering, those with intermediate distances are often sensitive to task order as described in Figure \ref{fig:order-sensitivity}.
% as in Figure {}: 예를 들어, Figure {}(a)의 예시에서 originally 3개의 task의 순서에 따라서 resulting number of groups가 달라짐

% for intermediate tasks
% Specifically, as a result of the assignment, i) a task with clearly large or small distance is directed to a newly-initialized semantic group to \textit{specifically} tune on a novel task or an existing semantic group, \textit{universally} tuned on previous similar tasks; ii) a task with intermediate semantic distance is allocated to a \textit{remergable} semantic group.
% As tasks progress, enriching our perspective on the CL environment, we perform a reassessment of the remergable group. This identifies tasks poised for universal applicability, amplifying overall generalizability.

% \min_{\theta_t, \phi} \ell_{ce} (f_\phi(f_{\theta_t}(x_t)), y_t) - \lambda {\rm Cosine}(q(x_t),\theta_t) 
% \min_{({\rm P}, {\rm k})\in\theta(t), \phi} \ell_{ce} (f_\phi(f_{P}(x_t)), y_t) - \gamma {\rm Cosine}() 
% OURS는 current task를 포함하는 sub-semantic groups에 대응되는 prompt parameters을 학습함.
% 이 prompts들은 하나씩 골라져서 Eq.(1)처럼 input tokens에 prepend되어 pre-trained model을 통과하게 됨.

% 이 prompt parmeters는 those corresponding to sub-semantic groups-{current_task}에서 copied and finetuned됨, additional knowledge being integrated without erasing the prior one.
% on the other hand, if no other elements in sub-semantic groups due to distinct semantics, prompt parameters are fully trained from scratch

% Overall, \algname minimizes the following loss function:
% train both prompts, keys, classification head 
% where classifer-head $f_\phi$, $f_p(t)$ the pre-trained architecture with prompts $p(t)$, l_ce, gamma. 
%  S(Gs) C(Gs)

% these sets of sub-semantic groups에서 

%  to implementation details?
% In terms of prompt tuning, novel semantic groups, which lack any relevant semantics, are fully trained from scratch while fine-tuning is adopted for existing semantics, ensuring that additional knowledge is integrated without erasing the prior one. 



% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=0.98\textwidth]{figures/model_arch.pdf}
%     % \caption{\textbf{ING}}
%     \vspace*{-0.3cm}
%     \caption{\textbf{Detailed view of the main components of \algname{}}: (a) drops the highly-activated features on the fused feature map according to the intensity $\kappa$; as in the example of the drop mask, the fusion facilitates identifying the background shortcuts from the signal of the high-level features on important parts such as the body of the dog. (b) adjusts the drop intensity $\kappa$ for the use in attentive debiasing. 
%     }
%     \label{fig:model_arch}
%     \vspace*{-0.2cm}
% \end{figure*}
% % Specifically, the coarse discriminative signals of the deep features pointing to a shortcut can be overlaid with essential parts, which should not be dropped.

% \noindent\textbf{Online Continual Learning.}
% We consider the online continual learning setting, where a sequence of tasks continually emerges with a set of new classes. Each data instance can be accessed only once unless it is stored in episodic memory. For the $t$-th task, let $D_t=\{(x^i_t,y^i_t)\}_{i=1}^{m_t}$ be a data stream obtained from a joint data distribution over $\mathcal{X}_t \times \mathcal{Y}_t$, where $\mathcal{X}_t$ is the input space, $\mathcal{Y}_t$ is the label space in a one-hot fashion, and $m_t$ is the number of instances of the $t$-th task. The goal of OCL is to train a classifier, such that it maximizes the test accuracy of all seen tasks $T=\{1,2, \dots, t\}$ at time $t$, with limited or no access to the data stream $D_{t^{\prime}}$ of previous tasks $t^{\prime}<t$.

% \medskip
% \noindent\textbf{Shortcut and Non-shortcut Features.}
% Let a DNN model trained on $(x,y) \sim \mathcal{X}\times\mathcal{Y}$ comprises a general feature extractor $f^{\theta}:\mathcal{X}\rightarrow\mathcal{Z}\in\mathbb{R}^d$ and a final classifier layer $g^{\text{w}}:\mathcal{Z}\rightarrow \mathbb{R}^{k}$, which is the multiplication of a linear weight matrix $\text{w}\in\mathbb{R}^{k\times d}$ and a feature $z\in \mathcal{Z}$ such that $g^{\text{w}}(z)=w\cdot z$. Here, $k$ is the number of classes, and $d$ is the dimensionality of a feature $z$. Let a \emph{feature} be the function mapping from the input space $\mathcal{X}$ to a real number; formally speaking, for the $i$-th sub-feature extractor of $f^{\theta}$ where $i\!\in\!\{1,2,\!\ldots\!,d\}$, $f^{\theta}_i:\mathcal{X}\rightarrow\mathbb{R}$. DNNs are known to have simplicity bias toward shortcut features which can easily distinguish between given classes\,\cite{geirhos2018imagenet, shah2020pitfalls, pezeshki2021gradient}. Then, the \emph{shortcut} and \emph{non-shortcut} features are defined by Definitions \ref{def:shortcut_feature} and \ref{def:non_shortcut_feature}, respectively.

% \begin{definition}{\sc (Shortcut Feature)}.
% Let $x$ and $\tilde{x}$ be the instances from seen and unseen data distributions $\mathcal{X}$ and $\mathcal{\tilde{X}}$, respectively, where $\mathcal{X}\cap\mathcal{\tilde{X}}=\emptyset$. We call a feature a \emph{shortcut} if it is not only highly activated ($\geq \rho$) for the seen data instance but also undesirably activated ($\geq \epsilon$) for the unseen data instance in expectation. That is,
% \vspace{-0.05cm}
% \begin{equation}
% f^{\theta}_{s}(\rho, \epsilon) : \mathbb{E}_{x \sim \mathcal{X}} \big[|f^{\theta}_s(x)| \big] \geq \rho ~\land ~ \mathbb{E}_{\tilde{x} \sim \mathcal{\tilde{X}}} \big[|f^{\theta}_s(\tilde{x})| \big] \geq \epsilon,
% \label{eq:shortcut_feature}
% \end{equation}
% where $s$ is the index of the shortcut feature. $\rho$ and $\epsilon$ are the thresholds indicating high activation for the seen and unseen data distributions. 
% \label{def:shortcut_feature}
% \vspace{-0.1cm}
% \end{definition}

% Note that a shortcut feature, e.g., an animal's legs, can be observed from the unseen instance, because it is not an intrinsic feature.

% \begin{definition}{\sc (Non-shortcut Feature)}.
% Let $x$ and $\tilde{x}$ be the instances from seen and unseen data distributions $\mathcal{X}$ and $\mathcal{\tilde{X}}$, respectively, where $\mathcal{X}\cap\mathcal{\tilde{X}}=\emptyset$. We call a feature a \emph{non-shortcut} if it is highly activated only for the seen instance in expectation. That is,
% \vspace{-0.05cm}
% \begin{equation}
% f^{\theta}_{n}(\rho, \epsilon) : \mathbb{E}_{x \sim \mathcal{X}} \big[|f^{\theta}_n(x)| \big] \geq \rho ~\land ~ \mathbb{E}_{\tilde{x} \sim \mathcal{\tilde{X}}} \big[|f^{\theta}_n(\tilde{x})| \big] < \epsilon. %\qed
% \label{eq:non_shortcut_feature}
% \end{equation}
% \label{def:non_shortcut_feature}
% \vspace{-0.7cm}
% \end{definition}

% \smallskip
% \noindent{\textbf{Property of Shortcut Feature.}} Due to a DNN's simplicity bias, the shortcut features tends to have higher activation values than the non-shortcut features\,\cite{shah2020pitfalls, pezeshki2021gradient}, such that
% \begin{equation}
% \mathbb{E}_{s\in \mathcal{S}} \big[|f^{\theta}_s(x)| \big]> \mathbb{E}_{n\in \mathcal{N}} \big[|f^{\theta}_n(x)| \big],
% \label{eq:shortcut_feature_property}
% \end{equation}
% where $\mathcal{S}$ and $\mathcal{N}$ are the set of the indices of shortcut and non-shortcut features, respectively.

% % ==========================================================================

% \section{Proposed Method: \algname{}}
% \label{sec:methodology}

% \algname{} realizes adaptive feature suppression thorough (a) \emph{attentive debiasing} with \emph{feature map fusion} and (b) \emph{adaptive intensity shifting}. The former drops high-attention features which are expected to be shortcuts, following the guidance from the latter in the form an adjusted drop intensity. Figure \ref{fig:model_arch} illustrates the detailed procedure of \algname{}. While (a) attentive debiasing is executed during the learning process, the drop intensity $\kappa$ is periodically adjusted by (b) adaptive intensity shifting. \algname{} can be implemented on top of any replay-based OCL methods, and see the implementation detail in Appendix A.


% \subsection{Attentive Debiasing}
% \label{subsec: Attentive Debiasing Layer}

% The shortcut features generally exhibit higher attention scores than the non-shortcut feature by Eq.\ \eqref{eq:shortcut_feature_property}. In addition, this shortcut bias usually appears as local or background cues\,\cite{scimeca2021shortcut}. Thus, after fusing the feature maps of different levels, we generate a \textrm{drop mask} to debias the effect of local or background cues on the feature activation.

% \smallskip
% \noindent{\textbf{Feature Map Fusion.}}
% The high-level features are essential to obtain discriminative signals, but they lack fine-grained details\,\cite{zhong2019shallow,wei2021shallow}, e.g., boundaries of objects. The low-level features embrace structural information with more details, which is helpful for accurately finding shortcut regions. Thus, feature map fusion is conducted to reduce the ambiguity in identifying the shortcut regions. Specifically, as shown in Figure \ref{fig:model_arch}(a), given a small memory footprint, we fuse the feature maps ${F}_{first}\in\mathbb{R}^{h\times w\times c}$ and ${F}_{last}$ $\in\mathbb{R}^{h^{\prime}\times w^{\prime}\times c^{\prime}}$ respectively from the first and last layers. To fuse the feature maps with different resolutions, i.e., $\langle {h, w, c}\rangle \neq \langle {h^{\prime}, w^{\prime}, c^{\prime} }\rangle$, the last layer's feature map $F_{last}$ is up-sampled to have the same resolution as the first layer's feature map $F_{first}$ such that $h^{\prime}=h$ and $w^{\prime}=w$. Then, we conduct average pooling along the channel dimension, compressing the outputs of all $c$ channels to produce the attention map ${A}_{fuse}$, which is formulated as
% \begin{equation}
% \begin{gathered}
% {F}_{fuse} = {F}_{first}\odot {\rm Upsample}({F}_{last})\in\mathbb{R}^{h\times w \times c}~~\text{and}\\
% {A}_{fuse} = {\rm ChannelPool}(F_{fuse})\in\mathbb{R}^{h\times w},
% \end{gathered}
% \label{eq:feature_fusion}
% \end{equation}
% where {\rm ChannelPool($\cdot$)} is the pooling along the channel, and $\odot$ is the element-wise tensor product.

% \smallskip
% \noindent{\textbf{Drop Mask Generation.}} 
% Given a drop intensity $\kappa\%$ for each class\footnote{The class is used only during the training process for debiasing. We do not perform such feature suppression in the middle of testing.}, we generate a \textit{drop mask} $M \in \mathbb{R}^{h \times w}$ based on the attention map ${A}_{fuse}$ in Eq.\ \eqref{eq:feature_fusion}. The mask at $(i,j)$ in $M$ is determined by
% \begin{equation}
% M_{i,j} =
% \begin{cases}
% 0 & \text{if}\!\!\quad (i,j) \in {\rm top\text{-}}\kappa(A_{fuse}) \\ 
% 1 & \text{otherwise},\\ 
% \end{cases}
% \label{eq:drop_mask}
% \end{equation}
% where ${\rm top\text{-}}\kappa(A_{fuse})$ returns the set of the top-$\kappa\%$ elements of $A_{fuse}$.
% %
% Last, we apply the drop mask to the first feature map ${F}_{first}$ after the stem layer of a backbone convolutional neural network\,(CNN), e.g., the feature map obtained by the first convolutional stem layer in ResNet18,
% \begin{equation}
% \Tilde{F}_{first} = M \odot {F}_{first}.
% \label{eq:drop_ops}
% \end{equation}
% This masking process affects all succeeding layers along the forward process. The masked feature map $\Tilde{F}_{first}$ accomplishes debiasing by using only the attention scores which can be computed on the fly.


% \subsection{Adaptive Intensity Shifting}
% \label{subsec: Adaptive Debiasing Intensity Scheduler}

% The extent of the shortcut bias naturally varies depending on the incoming tasks and the learning progress of a DNN model. Thus, \textit{adaptive intensity shifting} aims to guide {attentive debiasing} by adaptively adjusting the drop intensity $\kappa$ in a timely manner. The drop intensity is maintained separately for each class. It is \emph{decreased} if the removal of features is expected to lose important non-shortcut features which have high predictive power, \emph{increased} if the removal of features is expected to help emphasize important non-shortcut features, and \emph{unchanged} in neither of the cases,
% \begin{equation}
% \kappa \leftarrow \begin{cases}
% \kappa^\prime * \alpha & \text{if decrement} \\
% \kappa^\prime * (1/\alpha) & \text{if increment} \\
% \kappa^\prime & \text{otherwise},
% \end{cases}
% \label{eq:shifting}
% \end{equation}
% where $\kappa^\prime$ is the preceding value, and $\alpha$\,$(<1.0)$ is a hyperparameter that indicates the shift step.

% \smallskip
% \noindent{\textbf{Loss Collection.}} 
% To classify each case, we focus on the contribution to the reduction of the training loss because a better choice of the drop intensity leads to a better training performance\,\cite{scimeca2021shortcut, geirhos2020shortcut}. To determine whether a decrement or an increment is preferable, two potential values $\kappa=\kappa^\prime * \alpha$ and $\kappa=\kappa^\prime * (1/\alpha)$ alternate every $p$ iterations. The loss reductions are computed at the end of every $p$ iterations and maintained in the set $\mathcal{H}^{dec}$ when $\kappa^\prime * \alpha$ is used and in the set $\mathcal{H}^{inc}$ when $\kappa^\prime * (1/\alpha)$ is used, as shown in Figure \ref{fig:model_arch}(b),
% \begin{equation}
% \begin{gathered}
% \tiny
% \,\,\,{\mathcal{H}}^{dec} = \{\Delta\mathcal{L}_0,\Delta\mathcal{L}_{2p},\dots,\Delta\mathcal{L}_{2p(l-1)}\} \text{\small and} \\
% {\mathcal{H}}^{inc} = \{\underbrace{\Delta\mathcal{L}_{p},\Delta\mathcal{L}_{3p},\dots,\Delta\mathcal{L}_{2pl}}_{\text{Collect  } \Delta\mathcal{L} \text{  every  } 2p \text{  iterations}}\},
% \end{gathered}
% \end{equation}
% where $\Delta\mathcal{L}_{(q+1)\cdot p} = \mathcal{L}_{q\cdot p}-\mathcal{L}_{(q+1)\cdot p}$, and $\mathcal{L}_{(q+1) \cdot p}$ is the expected cross-entropy loss on the samples of a specific class in the memory buffer using the model at the iteration $(q+1)\cdot p$. Note that we compute the loss using the samples in the memory buffer rather than in a batch to obtain a more generalizable training loss. Those loss reductions are recorded until ${\mathcal{H}}^{dec}$ and ${\mathcal{H}}^{inc}$ have $l$ elements. Only a single model is needed to compare two shift directions, preserving the memory constraint of OCL.

% \smallskip
% \noindent{\textbf{Statistical Test and Update.}}
% When ${\mathcal{H}}^{dec}$ and ${\mathcal{H}}^{inc}$ become full every $2\cdot p \cdot l$ iterations, we conduct $t$-test to evaluate if one direction is statistically significant than the other with respect to the loss reduction, i.e., either $p$-value $\leq 0.05$ or $p$-value $\geq 0.95$. If a better direction exists, the preceding value is updated to the better direction; otherwise, it remains the same. Algorithm \ref{alg:pseudocode_adaptive_scheduler} describes the pseudocode of adaptive intensity shifting, which is self-explanatory.

% \input{figures/algorithm_adaptive_scheduler}

% \smallskip
% \noindent{\textbf{Training Data Stabilization.}}
% Furthermore, we consider the side effect of shifting the drop intensity during training. If it changes over time, the distribution of input features could be swayed inconsistently. As widely claimed in \cite{ioffe2015batch, zhou2022online}, this problem often causes training instability and eventually deteriorates the overall performance. In this sense, we decide to drop $\gamma\%$ of the features \emph{constantly}. Thus, $\kappa$ cannot grow beyond $\gamma$; if $\kappa < \gamma$, $(\gamma-\kappa)$\% of the features are additionally chosen uniformly at random among those whose drop mask is not $1$.


% \subsection{Understanding of Shortcut Bias in OCL}
% \label{sec:theoretical_analysis}

% From a theoretical standpoint, we clarify two detrimental effects of learning shortcut features in OCL. See Appendix B for relevant empirical evidences. Let $g^{\text{w}}_i:\mathbb{R}\rightarrow\mathbb{R}^{k}$ be the multiplication of an $i$-th column vector of the weight matrix $\text{w}$ and an $i$-th feature $f_i^\theta$. Then, $g^{\text{w}}_i(f^{\theta}_i(x))$ denotes the contribution of the $i$-th feature to a prediction, i.e., how much the $i$-th feature $f^{\theta}_i(x)$ contributes to the prediction $g^{\text{w}}(f^{\theta}(x))$, since $g^{\text{w}}(f^{\theta}(x))= \sum_{i=1}^d{g^{\text{w}}_i(f^{\theta}_i(x))}$. Here, we formulate low transferability and high forgetability of shortcut features in OCL.

% \begin{property}[{\sc Low Transferability}]
% A shortcut feature of the current task hinders the model from learning the knowledge of the next task.
% \end{property}
% \begin{proof}
% Let's consider training a classifier for the ($t$+1)-th task, given a shortcut biased model $\theta_t$ as the initial model. By Eq.~\eqref{eq:shortcut_feature}, $\mathbb{E}_{x_{t+1} \sim \mathcal{X}_{t+1}}\big[|f^{\theta_t}_s(x_{t+1})| \big] \geq \epsilon$ if $x_{t+1}$ shares the same shortcut features with $x_t$. Then, when training a new model $\theta_{t+1}$ from the model $\theta_{t}$, the shortcut feature $f^{\theta_t}_s$ is no longer discriminative since it can appear in both $\mathcal{X}_{t}$ and $\mathcal{X}_{t+1}$. Thus, the model $\theta_{t+1}$ should learn a totally new discriminative feature, meaning that the model $\theta_{t+1}$  starts from a poor initialization. As a result, the training convergence becomes slower compared with a non-biased model $\theta_t^*$.
% \end{proof}

% \begin{property}[{\sc High Forgetability}]
% A shortcut feature of the current task makes the model forget the knowledge of the previous tasks.
% \end{property}
% \begin{proof}
% Given the previous tasks at $t^{\prime}\in\{1,\ldots,t-1\}$ and the current task at $t$, let's assume that we trained a shortcut biased classifier $\theta_t$.
% Then, the shortcut feature $s$ of $f^{\theta_t}$ contributes to predict the class $y_t\in\mathcal{Y}_t$ such that $\argmax g^{\text{w}_t}_s(f^{\theta_t}_s(x_t))=y_t\in\mathcal{Y}_t$. However, by Eq.~\eqref{eq:shortcut_feature}, $\mathbb{E}_{x_{t^{\prime}} \sim \mathcal{X}_{t^{\prime}}}\big[|f^{\theta_t}_s(x_{t^{\prime}})| \big] \geq \epsilon$ if $x_{t^{\prime}}$ shares the same shortcut features with $x_{t}$.
% Then, even for the previous instance $x_{t^{\prime}}$, the shortcut feature $s$ contributes to predict the class $y_{t}\in\mathcal{Y}_{t}$ such that $\argmax g^{\text{w}_t}_s(f^{\theta_t}_s(x_{t^{\prime}}))=y_t\notin\mathcal{Y}_{t^{\prime}}$, which is a wrong prediction.
% Due to the high activation of shortcut features in Eq.~\eqref{eq:shortcut_feature_property}, this wrong feature contribution gives a significant impact to the final prediction $g^{\text{w}}(f^{\theta}(x_{t^{\prime}}))= \sum_{i=1}^d{g^{\text{w}}_i(f^{\theta}_i(x_{t^{\prime}}))}$, so that the model highly forgets the knowledge of the previous tasks. 
% \end{proof}




% % \subsection{Empirical Proofs of Two Properties}
% % \label{sec:empirical_shorcut_bias_ocl}

% % \begin{figure}[!t]
% %     \centering
% %     \includegraphics[width=0.9\columnwidth]{figures/preliminary_two.pdf}
% %     \hspace{2cm} \small (a) Transferability. \hspace{1.5cm} (b) Forgetability
% %     \vspace{-0.1cm}
% %     \caption{(a) shows lower transferability and (b) shows higher forgetting of shortcut features compared to non-shortcut features.
% %     %(a) shows low transferability in learning task 2 of B-MNIST\,(green 2 and 3) and (b) represents strong forgetting in task 1 after learning task 2 of B-MNIST\,(red 2 and green 3).
% % }
% %     \label{fig:preliminary_exp}
% % \end{figure}

% % %\subsection{Shortcut Induced Performance Degradation}
% % %\label{subsec:preliminary-exp}

% % %\smallskip\smallskip\noindent{\textbf{Experiment setup.}} 
% % To empricially investigate the aforementioned two properties, we conduct a simple controlled experiment using two datasets; MNIST\,\cite{lecun1998gradient} and Biased MNIST (B-MNIST)\,\cite{bahng2020learning}, which is widely utilized in bias learning~\cite{bahng2020learning,bui2021exploiting,tartaglione2021end}.
% % In B-MNIST, each digit is on a different colored background; 0 on red and 1 on green.
% % DNNs trained on B-MNIST employ only color shortcut features for classification because color is a simpler feature than shape of digits.
% % We train ER\,\cite{rolnick2019experience} for OCL setup with two tasks--- Task 1 (T1): classify 0 and 1, and Task 2 (T2): classify 2 and 3.
% % % How to expose color bias on B-MNIST?

% % \smallskip\noindent{\textbf{Low Transferability.}}
% % To validate the transferability, we designate the background color for T2 of B-MNIST as green for both digits 2 and 3.
% % Figure \ref{fig:preliminary_exp}(a) shows the lower transferability of shortcut features than that of non-shortcut features.
% % When training T2, ER trained on B-MNIST (the shortcut biased model) shows slower increase of test accuracy than ER trained on MNIST, since red and green color features learned in T1 are not helpful to generalize well in T2.
% % This indicates that the transferability of the OCL model significantly deteriorates once the model is biased to the shortcut features.

% % \smallskip\noindent{\textbf{High Foregetability.}}
% % To validate the forgetability, we designate the background color for T2 of B-MNIST as green for digit 2 and red for digit 3.
% % Figure \ref{fig:preliminary_exp}(b) shows the higher forgetability of shortcut features than that of non-shortcut features.
% % After training task 2, ER trained on B-MNIST shows rapid forgetting of the class prediction in T1, since the red or green color becomes a shortcut cue to predict the digit 2 or 3 in T2.
% % This indicates that the OCL model also be significantly threatened by forgetting once the model is biased to the shortcut features.


% \begin{comment}
% The empirical results in Figure \ref{fig:preliminary_exp} support the underlying claim that the adverse effect of shortcut learning to transferability and forgetting. The experiments were conducted on sequential Biased MNIST\,(B-MNIST)\,\cite{bahng2020learning} where different colors are designated for each digit as shortcut. 
% The accuracy of a widely applied OCL method, ER\,\cite{rolnick2019experience}, trained on B-MNIST in Figure \ref{fig:preliminary_exp}(a) shows shortcut bias on color while overlooking shape of digits.
% As in Figure \ref{fig:preliminary_exp}(b), stronger forgetting is observed in the model biased on shortcut when the color feature is no longer discriminative for classifying the first task. The model with color bias also suffers from lower transferability and we speculate that the color bias does not generalize well to unseen new classes, as in Figure \ref{fig:preliminary_exp}(c).
% % learns the semantically dissimilar task\,(e.g., classifying two same color digits) requiring a feature\,(e.g., shape) other than color, as in Figure \ref{fig:preliminary_exp}(c).
% \end{comment}

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> tables/ablation_refining_effect.tex <==
% \newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \bgroup
\def\arraystretch{1.1}% make the row margin compact
\begin{table}[t]
\small
% \tiny
% \scriptsize
% \small
% \label{tbl:RegionBuzComparison}
\centering
% \vspace*{-0.3cm}
\caption{
Ablation analysis highlighting the impact of semantic refinement and prospective prompt tuning on $A_{last}$. The highest values are emphasized in bold. }
\vspace*{0.2cm}
\resizebox{0.90\linewidth}{!}{%
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
% {@{}c|c||C{0.9cm}C{1.1cm}||C{0.9cm}c@{}}
% {@{}c||C{1.1cm}|C{1.2cm}|C{1.2cm}|C{1.1cm}c@{}}
{@{}l||c|c|cc@{}}
\toprule
% \multicolumn{1}{c||}{} & \multicolumn{3}{c|}{\textbf{{    Variants   }}} & \multicolumn{1}{c}{} \\\cline{2-4}
% \multicolumn{1}{c||}{\textbf{}} & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{No Drop Int. Shift}} & \multicolumn{1}{c}{} \\
% \smallskip
\multicolumn{1}{c||}{{Shifting Scenarios}} %\hspace{-0.3cm}\textbf{Method}}
& \multicolumn{1}{c|}{\textbf{No Refine}}
& \multicolumn{1}{c|}{\textbf{Avg Merge}}
& \multicolumn{1}{c}{\textbf{\algname{}}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
% & \multicolumn{1}{c|}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
% & \multicolumn{1}{c|}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
% & \multicolumn{1}{c}{\bm{$A_{avg}$}}

\\ \toprule
% # Mild ###############################################################
\multirow{1}{*}{\textbf{Mild}\,\scalebox{0.80}{(ImageNet-R)}}                                
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{85.31}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{85.31}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{85.31}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\textbf{45.5}}\end{tabular}
\\
% \midrule
% \cdashline{}
% # ER ###############################################################


% DER ++ ###############################################################
\multirow{1}{*}{\textbf{Moderate}\,\scalebox{0.80}{(VTAB-Rec10)}}                                         
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{51.80}\scalebox{0.99}\,($\pm$0.62)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{52.92}\scalebox{0.99}\,($\pm$1.06)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{54.22}}\scalebox{0.99}\,($\pm$0.52)\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\textbf{44.4}}\end{tabular}
\\
% \midrule
% % # ++ ###############################################################

% # MIR ################################################################
\multirow{1}{*}{\textbf{Abrupt}\,\scalebox{0.80}{(VTAB-19T)}}                                                    
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{31.25}\scalebox{0.99}\,($\pm$0.20)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{30.08}\scalebox{0.99}\,($\pm$0.26)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{32.39}}\scalebox{0.99}\,($\pm$0.32)\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{{38.7}}\end{tabular}
\\
\midrule
% \cdashline{}
\multirow{1}{*}{{\textit{Average Degradation.}}\hspace{-0.15cm}}            
& \begin{tabular}[c]{@{}c@{}}{{2.8\%}\hspace{-1cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{3.4\%}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{-}}\end{tabular}
\\
\bottomrule
\end{tabular} }
\label{tbl:ablation}
\end{table}
% 54.225

==> tables/overall_perf.tex <==
%\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \bgroup
\def\arraystretch{1.25}% make the row margin compact
\begin{table*}[t!]
\small
% \tiny
% \scriptsize
% \small
\centering
%\vspace*{-0.2cm}
\caption{Performance comparison of \algname{} against CL baselines using prompt tuning across uniformly and dynamically shifting scenarios. This assesses last accuracy\,(higher preferred) and forgetting\,(lower preferred), in addition to the average improvements and number of semantic groups by \algname{}. We report the average relative improvements over the most effective universal\,(LAE) and specific\,(S-Prompts) prompting methods. The best and second-best values are highlighted in bold and underlined, respectively.}
\vspace*{0.25cm}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
% {@{}c|c||C{1.85cm}c|C{1.85cm}c|C{1.85cm}cc@{}}
{@{}cc|c|ccccc|cccc@{}}
\toprule
\multirow{2}{*}{\hspace{-0.0cm}\makecell[c]{Shifting\\Scenarios}\hspace{-0.0cm}}&\multirow{2}{*}{\makecell[c]{CL\\Datasets}} &\multirow{2}{*}{\makecell[c]{Metrics}}
& \multicolumn{5}{c|}{{ {Prompt Tuning CL Algorithms}}} 
& \multicolumn{3}{c}{{ {\algname{} }}}\\%\cline{3-14} 

& & & \multicolumn{1}{c}{\hspace{-0.0cm}{L2P}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{VPT}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{LAE}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{DP}}
& \multicolumn{1}{c|}{\hspace{-0.01cm}{S-Prompts}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{\algname{}}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{\textit{Avg. Improv.}}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{\textit{\#Semantics}}}
\\ \midrule

% # Mild ###############################################################
\multirow{4}{*}{\hspace{-0.0cm}{\textbf{Mild}}\hspace{-0.01cm}} 
& \multirow{2}{*}{\makecell[c]{ImageNet-R}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{68.05}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{69.31}\scalebox{0.99}\,($\pm$0.09)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{70.11}}\scalebox{0.99}\,($\pm$0.12)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{67.81}\scalebox{0.99}\,($\pm$0.19)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{65.89}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{69.45}}\scalebox{0.99}\,({$\pm$0.14})\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{2.13}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{1.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.17}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.27}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.05}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.99}}\scalebox{0.99}\,($\pm$0.18)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.71}\scalebox{0.99}\,($\pm$0.22)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.94}}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{28.2}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{CIFAR100}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{84.55}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{85.34}}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{85.16}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{84.79}\scalebox{0.99}\,($\pm$0.14)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{83.73}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{85.31}}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{1.02}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{1.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{5.59}}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.19}\scalebox{0.99}\,($\pm$0.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.05}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{5.04}}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.41}\scalebox{0.99}\,($\pm$0.13)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.21}\scalebox{0.99}\,($\pm$0.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{0.32}}\%\hspace{-0.01cm} }\end{tabular}
% & \multirow{2}{*}{\makecell[c]{1.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\
\midrule
\multirow{13}{*}{\hspace{-0.0cm}{\textbf{Moderate}}\hspace{-0.01cm}} 
& \multirow{2}{*}{\makecell[c]{VTAB-Sim25}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.28}\scalebox{0.99}\,($\pm$0.50)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.24}\scalebox{0.99}\,($\pm$0.57)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.57}\scalebox{0.99}\,($\pm$0.72)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.72}\scalebox{0.99}\,($\pm$0.60)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.72}}\scalebox{0.99}\,($\pm$0.40)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{39.56}}\scalebox{0.99}\,($\pm$0.59)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{3.71}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{16.4}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}16.4\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{6.73}}\scalebox{0.99}\,($\pm$0.79)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.23}\scalebox{0.99}\,($\pm$0.65)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{9.51}\scalebox{0.99}\,($\pm$0.87)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{6.90}}\scalebox{0.99}\,($\pm$0.88)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.11}\scalebox{0.99}\,($\pm$0.53)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.10}\scalebox{0.99}\,($\pm$0.73)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{14.56}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}16.4\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Sim50}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.14}\scalebox{0.99}\,($\pm$0.36)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.30}\scalebox{0.99}\,($\pm$0.50)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.85}\scalebox{0.99}\,($\pm$0.73)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.22}\scalebox{0.99}\,($\pm$0.53)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.97}}\scalebox{0.99}\,($\pm$0.51)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{39.27}}\scalebox{0.99}\,($\pm$0.51)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{2.24}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{13.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}13.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.53}\scalebox{0.99}\,($\pm$0.71)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.22}\scalebox{0.99}\,($\pm$0.57)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.02}\scalebox{0.99}\,($\pm$0.54)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.98}}\scalebox{0.99}\,($\pm$0.49)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.72}}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.77}\scalebox{0.99}\,($\pm$0.65)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{1.70}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}13.0\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Sim75}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.17}\scalebox{0.99}\,($\pm$0.76)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.53}}\scalebox{0.99}\,($\pm$0.73)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.55}\scalebox{0.99}\,($\pm$0.82)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.39}\scalebox{0.99}\,($\pm$0.78)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.86}\scalebox{0.99}\,($\pm$0.63)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{39.55}}\scalebox{0.99}\,($\pm$0.46)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{4.89}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{12.2}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}12.2\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{3.53}\scalebox{0.99}\,($\pm$0.27)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{3.26}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.88}\scalebox{0.99}\,($\pm$0.24)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{3.17}}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{3.16}}\scalebox{0.99}\,($\pm$0.31)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{3.42}\scalebox{0.99}\,($\pm$0.31)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{24.34}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}12.2\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Rec2}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{52.05}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{51.97}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{54.68}}\scalebox{0.99}\,($\pm$0.19)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{51.65}\scalebox{0.99}\,($\pm$0.06)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{53.52}\scalebox{0.99}\,($\pm$0.41)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{54.88}}\scalebox{0.99}\,($\pm$0.27)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{1.44}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{5.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.2\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.67}\scalebox{0.99}\,($\pm$2.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.40}\scalebox{0.99}\,($\pm$2.27)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{10.74}\scalebox{0.99}\,($\pm$1.76)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.81}\scalebox{0.99}\,($\pm$2.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{6.54}}\scalebox{0.99}\,($\pm$1.20)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{7.49}}\scalebox{0.99}\,($\pm$2.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{13.31}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.2\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Rec5}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 

& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{53.98}}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{53.45}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{53.45}\scalebox{0.99}\,($\pm$0.31)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{53.85}\scalebox{0.99}\,($\pm$0.18)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{52.80}\scalebox{0.99}\,($\pm$0.17)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{56.08}}\scalebox{0.99}\,($\pm$0.59)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{5.56}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{5.8}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.4\hspace{-0.01cm} }\end{tabular}
\\ 
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.49}}\scalebox{0.99}\,($\pm$0.68)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.03}}\scalebox{0.99}\,($\pm$0.67)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.41}\scalebox{0.99}\,($\pm$0.56)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.66}\scalebox{0.99}\,($\pm$0.68)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.27}\scalebox{0.99}\,($\pm$0.49)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.03}\scalebox{0.99}\,($\pm$0.47)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{13.87}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.4\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Rec10}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{52.20}\scalebox{0.99}\,($\pm$0.81)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{51.70}\scalebox{0.99}\,($\pm$0.44)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{52.34}}\scalebox{0.99}\,($\pm$0.35)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{50.80}\scalebox{0.99}\,($\pm$0.58)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{47.72}\scalebox{0.99}\,($\pm$0.20)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{54.22}}\scalebox{0.99}\,($\pm$0.52)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{8.37}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.6\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{6.2}}
\\ 
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.33}\scalebox{0.99}\,($\pm$0.37)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.25}\scalebox{0.99}\,($\pm$0.53)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.87}\scalebox{0.99}\,($\pm$0.43)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.07}\scalebox{0.99}\,($\pm$0.46)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.00}\scalebox{0.99}\,($\pm$0.52)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.32}\scalebox{0.99}\,($\pm$0.62)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{-4.85}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.6\hspace{-0.01cm} }\end{tabular}
\\ \midrule
\multirow{4}{*}{\hspace{-0.0cm}{\textbf{Abrupt}}\hspace{-0.01cm}} 
& \multirow{2}{*}{\makecell[c]{VTAB-19T}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{28.23}\scalebox{0.99}\,($\pm$0.14)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{28.11}\scalebox{0.99}\,($\pm$0.20)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{26.71}\scalebox{0.99}\,($\pm$0.29)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{28.48}\scalebox{0.99}\,($\pm$0.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{30.83}}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{32.39}}\scalebox{0.99}\,($\pm$0.32)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{12.58}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{18.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}18.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.15}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.43}\scalebox{0.99}\,($\pm$0.55)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{9.48}\scalebox{0.99}\,($\pm$0.54)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.50}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.01}}\scalebox{0.99}\,($\pm$0.23)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.30}}\scalebox{0.99}\,($\pm$0.69)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{36.25}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}18.0\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-5T}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{34.31}\scalebox{0.99}\,($\pm$0.04)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{34.03}\scalebox{0.99}\,($\pm$0.05)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{35.30}\scalebox{0.99}\,($\pm$0.41)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{34.17}\scalebox{0.99}\,($\pm$0.04)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.27}}\scalebox{0.99}\,($\pm$0.18)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{38.67}}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{5.12}}\%\hspace{-0.01cm} }\end{tabular}
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}5.0\end{tabular}}
& \multirow{2}{*}{\makecell[c]{5.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.55}\scalebox{0.99}\,($\pm$1.13)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.88}\scalebox{0.99}\,($\pm$1.09)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{17.72}\scalebox{0.99}\,($\pm$1.29)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.57}\scalebox{0.99}\,($\pm$1.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{12.84}}\scalebox{0.99}\,($\pm$0.98)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{13.25}}\scalebox{0.99}\,($\pm$1.00)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{13.29}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.0\hspace{-0.01cm} }\end{tabular}
\\
\bottomrule
\end{tabular}
}
\label{tbl:overall_perf}
% \vspace{-0.5cm}
\end{table*}


==> tables/overall_perf_noshuf.tex <==
%\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \bgroup
\def\arraystretch{1.25}% make the row margin compact
\begin{table*}[t!]
\small
% \tiny
% \scriptsize
% \small
\centering
%\vspace*{-0.2cm}
\caption{Comparative performance of \algname{} versus prompt tuning-based CL baselines in mild, moderate, and abrupt shifting scenarios. This assesses last accuracy (higher preferred) and forgetting (lower preferred), along with the number of semantic groups by \algname{} for each scenario. The best and second-best performances for each metric are highlighted in bold and underlined, respectively.}
\vspace*{0.25cm}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
% {@{}c|c||C{1.85cm}c|C{1.85cm}c|C{1.85cm}cc@{}}
{@{}cc|c|ccccc|cccc@{}}
\toprule
\multirow{2}{*}{\hspace{-0.0cm}\makecell[c]{Shifting\\Scenarios}\hspace{-0.0cm}}&\multirow{2}{*}{\makecell[c]{CL\\Datasets}} &\multirow{2}{*}{\makecell[c]{Metrics}}
& \multicolumn{5}{c|}{{ {Prompt Tuning CL Algorithms}}} 
& \multicolumn{3}{c}{{ {\algname{} }}}\\%\cline{3-14} 

& & & \multicolumn{1}{c}{\hspace{-0.0cm}{L2P}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{VPT}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{LAE}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{DP}}
& \multicolumn{1}{c|}{\hspace{-0.01cm}{S-Prompts}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{\algname{}}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{\textit{Avg. Improv.}}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{\textit{\#Semantics}}}
\\ \midrule

% # Mild ###############################################################
\multirow{4}{*}{\hspace{-0.0cm}{\textbf{Mild}}\hspace{-0.01cm}} 
& \multirow{2}{*}{\makecell[c]{ImageNet-R}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{68.05}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{69.31}\scalebox{0.99}\,($\pm$0.09)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{70.11}}\scalebox{0.99}\,($\pm$0.12)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{67.81}\scalebox{0.99}\,($\pm$0.19)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{65.89}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{69.45}}\scalebox{0.99}\,({$\pm$0.14})\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{1.78}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{1.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.17}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.27}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.05}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.99}}\scalebox{0.99}\,($\pm$0.18)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.71}\scalebox{0.99}\,($\pm$0.22)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.94}}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{15.38}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{CIFAR100}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{84.55}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{85.34}}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{85.16}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{84.79}\scalebox{0.99}\,($\pm$0.14)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{83.73}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{85.31}}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{0.70}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{1.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{5.59}}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.19}\scalebox{0.99}\,($\pm$0.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.05}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{5.04}}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.41}\scalebox{0.99}\,($\pm$0.13)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.21}\scalebox{0.99}\,($\pm$0.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{-6.05}}\%\hspace{-0.01cm} }\end{tabular}
% & \multirow{2}{*}{\makecell[c]{1.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\
\midrule
\multirow{13}{*}{\hspace{-0.0cm}{\textbf{Moderate}}\hspace{-0.01cm}} 
& \multirow{2}{*}{\makecell[c]{VTAB-Sim25}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.28}\scalebox{0.99}\,($\pm$0.50)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.24}\scalebox{0.99}\,($\pm$0.57)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.57}\scalebox{0.99}\,($\pm$0.72)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.72}\scalebox{0.99}\,($\pm$0.60)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.72}}\scalebox{0.99}\,($\pm$0.40)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{39.56}}\scalebox{0.99}\,($\pm$0.59)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{3.82}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{16.4}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}16.4\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{6.73}}\scalebox{0.99}\,($\pm$0.79)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.23}\scalebox{0.99}\,($\pm$0.65)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{9.51}\scalebox{0.99}\,($\pm$0.87)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{6.90}}\scalebox{0.99}\,($\pm$0.88)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.11}\scalebox{0.99}\,($\pm$0.53)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.10}\scalebox{0.99}\,($\pm$0.73)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{5.28}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}16.4\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Sim50}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.14}\scalebox{0.99}\,($\pm$0.36)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.30}\scalebox{0.99}\,($\pm$0.50)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.85}\scalebox{0.99}\,($\pm$0.73)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.22}\scalebox{0.99}\,($\pm$0.53)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.97}}\scalebox{0.99}\,($\pm$0.51)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{39.27}}\scalebox{0.99}\,($\pm$0.51)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{2.54}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{13.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}13.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.53}\scalebox{0.99}\,($\pm$0.71)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.22}\scalebox{0.99}\,($\pm$0.57)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.02}\scalebox{0.99}\,($\pm$0.54)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.98}}\scalebox{0.99}\,($\pm$0.49)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.72}}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.77}\scalebox{0.99}\,($\pm$0.65)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{-5.02}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}13.0\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Sim75}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.17}\scalebox{0.99}\,($\pm$0.76)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.53}}\scalebox{0.99}\,($\pm$0.73)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.55}\scalebox{0.99}\,($\pm$0.82)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.39}\scalebox{0.99}\,($\pm$0.78)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.86}\scalebox{0.99}\,($\pm$0.63)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{39.55}}\scalebox{0.99}\,($\pm$0.46)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{3.81}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{12.2}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}12.2\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{3.53}\scalebox{0.99}\,($\pm$0.27)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{3.26}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.88}\scalebox{0.99}\,($\pm$0.24)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{3.17}}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{3.16}}\scalebox{0.99}\,($\pm$0.31)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{3.42}\scalebox{0.99}\,($\pm$0.31)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{10.00}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}12.2\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Rec2}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{52.32}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{53.22}}\scalebox{0.99}\,($\pm$0.44)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{51.22}\scalebox{0.99}\,($\pm$0.40)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{51.75}\scalebox{0.99}\,($\pm$0.13)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{52.85}\scalebox{0.99}\,($\pm$0.32)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{55.47}}\scalebox{0.99}\,($\pm$0.09)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{6.12}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{5.2}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.2\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{11.46}}\scalebox{0.99}\,($\pm$2.20)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{11.31}}\scalebox{0.99}\,($\pm$2.13)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.28}\scalebox{0.99}\,($\pm$2.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{11.72}\scalebox{0.99}\,($\pm$2.13)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{12.22}\scalebox{0.99}\,($\pm$2.14)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{11.51}\scalebox{0.99}\,($\pm$1.99)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{7.16}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.2\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Rec5}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{53.70}\scalebox{0.99}\,($\pm$0.75)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{54.35}}\scalebox{0.99}\,($\pm$1.41)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{50.85}\scalebox{0.99}\,($\pm$0.69)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{52.65}\scalebox{0.99}\,($\pm$0.90)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{52.10}\scalebox{0.99}\,($\pm$0.32)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{57.42}}\scalebox{0.99}\,($\pm$0.82)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{8.89}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{5.4}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.4\hspace{-0.01cm} }\end{tabular}
\\ 
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{13.65}\scalebox{0.99}\,($\pm$1.76)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{13.70}\scalebox{0.99}\,($\pm$1.58)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.07}\scalebox{0.99}\,($\pm$1.94)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{13.36}\scalebox{0.99}\,($\pm$1.59)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{11.91}}\scalebox{0.99}\,($\pm$1.79)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{12.08}}\scalebox{0.99}\,($\pm$1.53)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{10.77}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.4\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Rec10}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{48.82}\scalebox{0.99}\,($\pm$0.66)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{51.55}}\scalebox{0.99}\,($\pm$0.24)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{47.75}\scalebox{0.99}\,($\pm$0.25)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{51.20}\scalebox{0.99}\,($\pm$0.52)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{45.92}\scalebox{0.99}\,($\pm$0.89)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{53.08}}\scalebox{0.99}\,($\pm$0.76)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{8.22}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.6\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{5.6}}
\\ 
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.79}\scalebox{0.99}\,($\pm$1.01)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{16.60}\scalebox{0.99}\,($\pm$0.97)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{17.43}\scalebox{0.99}\,($\pm$1.25)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{14.70}}\scalebox{0.99}\,($\pm$1.04)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{16.15}\scalebox{0.99}\,($\pm$1.82)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{15.51}}\scalebox{0.99}\,($\pm$1.04)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{3.87}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.6\hspace{-0.01cm} }\end{tabular}
\\ \midrule
\multirow{4}{*}{\hspace{-0.0cm}{\textbf{Abrupt}}\hspace{-0.01cm}} 
& \multirow{2}{*}{\makecell[c]{VTAB-19T}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{28.23}\scalebox{0.99}\,($\pm$0.14)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{28.11}\scalebox{0.99}\,($\pm$0.20)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{26.71}\scalebox{0.99}\,($\pm$0.29)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{28.48}\scalebox{0.99}\,($\pm$0.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{30.83}}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{32.39}}\scalebox{0.99}\,($\pm$0.32)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{13.76}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{18.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}18.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.15}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.43}\scalebox{0.99}\,($\pm$0.55)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{9.48}\scalebox{0.99}\,($\pm$0.54)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.50}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.01}}\scalebox{0.99}\,($\pm$0.23)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.30}}\scalebox{0.99}\,($\pm$0.69)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{31.90}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}18.0\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-5T}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{34.31}\scalebox{0.99}\,($\pm$0.04)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{34.03}\scalebox{0.99}\,($\pm$0.05)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{35.30}\scalebox{0.99}\,($\pm$0.41)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{34.17}\scalebox{0.99}\,($\pm$0.04)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.27}}\scalebox{0.99}\,($\pm$0.18)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{38.67}}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{9.81}}\%\hspace{-0.01cm} }\end{tabular}
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}5.0\end{tabular}}
& \multirow{2}{*}{\makecell[c]{5.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.55}\scalebox{0.99}\,($\pm$1.13)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.88}\scalebox{0.99}\,($\pm$1.09)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{17.72}\scalebox{0.99}\,($\pm$1.29)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.57}\scalebox{0.99}\,($\pm$1.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{12.84}}\scalebox{0.99}\,($\pm$0.98)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{13.25}}\scalebox{0.99}\,($\pm$1.00)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{14.58}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.0\hspace{-0.01cm} }\end{tabular}
\\
\bottomrule
\end{tabular}
}
\label{tbl:overall_perf}
% \vspace{-0.5cm}
\end{table*}


==> tables/overall_perf_shuf.tex <==
%\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \bgroup
\def\arraystretch{1.25}% make the row margin compact
\begin{table*}[t!]
\small
% \tiny
% \scriptsize
% \small
\centering
%\vspace*{-0.2cm}
\caption{Comparative performance of \algname{} versus prompt tuning-based CL baselines in mild, moderate, and abrupt shifting scenarios. This assesses last accuracy (higher preferred) and forgetting (lower preferred), along with the number of semantic groups by \algname{} for each scenario. The best and second-best performances for each metric are highlighted in bold and underlined, respectively.}
\vspace*{0.25cm}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
% {@{}c|c||C{1.85cm}c|C{1.85cm}c|C{1.85cm}cc@{}}
{@{}cc|c|ccccc|cccc@{}}
\toprule
\multirow{2}{*}{\hspace{-0.0cm}\makecell[c]{Shifting\\Scenarios}\hspace{-0.0cm}}&\multirow{2}{*}{\makecell[c]{CL\\Datasets}} &\multirow{2}{*}{\makecell[c]{Metrics}}
& \multicolumn{5}{c|}{{ {Prompt Tuning CL Algorithms}}} 
& \multicolumn{3}{c}{{ {\algname{} }}}\\%\cline{3-14} 

& & & \multicolumn{1}{c}{\hspace{-0.0cm}{L2P}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{VPT}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{LAE}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{DP}}
& \multicolumn{1}{c|}{\hspace{-0.01cm}{S-Prompts}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{\algname{}}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{\textit{Avg. Improv.}}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{\textit{\#Semantics}}}
\\ \midrule

% # Mild ###############################################################
\multirow{4}{*}{\hspace{-0.0cm}{\textbf{Mild}}\hspace{-0.01cm}} 
& \multirow{2}{*}{\makecell[c]{ImageNet-R}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{68.05}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{69.31}\scalebox{0.99}\,($\pm$0.09)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{70.11}}\scalebox{0.99}\,($\pm$0.12)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{67.81}\scalebox{0.99}\,($\pm$0.19)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{65.89}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{69.45}}\scalebox{0.99}\,({$\pm$0.14})\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{1.78}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{1.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.17}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.27}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.05}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.99}}\scalebox{0.99}\,($\pm$0.18)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.71}\scalebox{0.99}\,($\pm$0.22)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.94}}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{15.38}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{CIFAR100}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{84.55}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{85.34}}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{85.16}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{84.79}\scalebox{0.99}\,($\pm$0.14)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{83.73}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{85.31}}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{0.70}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{1.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{5.59}}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.19}\scalebox{0.99}\,($\pm$0.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.05}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{5.04}}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.41}\scalebox{0.99}\,($\pm$0.13)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.21}\scalebox{0.99}\,($\pm$0.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{-6.05}}\%\hspace{-0.01cm} }\end{tabular}
% & \multirow{2}{*}{\makecell[c]{1.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\
\midrule
\multirow{13}{*}{\hspace{-0.0cm}{\textbf{Moderate}}\hspace{-0.01cm}} 
& \multirow{2}{*}{\makecell[c]{VTAB-Sim25}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.28}\scalebox{0.99}\,($\pm$0.50)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.24}\scalebox{0.99}\,($\pm$0.57)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.57}\scalebox{0.99}\,($\pm$0.72)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.72}\scalebox{0.99}\,($\pm$0.60)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.72}}\scalebox{0.99}\,($\pm$0.40)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{39.56}}\scalebox{0.99}\,($\pm$0.59)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{3.82}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{16.4}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}16.4\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{6.73}}\scalebox{0.99}\,($\pm$0.79)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.23}\scalebox{0.99}\,($\pm$0.65)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{9.51}\scalebox{0.99}\,($\pm$0.87)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{6.90}}\scalebox{0.99}\,($\pm$0.88)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.11}\scalebox{0.99}\,($\pm$0.53)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.10}\scalebox{0.99}\,($\pm$0.73)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{5.28}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}16.4\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Sim50}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.14}\scalebox{0.99}\,($\pm$0.36)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.30}\scalebox{0.99}\,($\pm$0.50)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.85}\scalebox{0.99}\,($\pm$0.73)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.22}\scalebox{0.99}\,($\pm$0.53)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.97}}\scalebox{0.99}\,($\pm$0.51)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{39.27}}\scalebox{0.99}\,($\pm$0.51)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{2.54}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{13.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}13.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.53}\scalebox{0.99}\,($\pm$0.71)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.22}\scalebox{0.99}\,($\pm$0.57)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.02}\scalebox{0.99}\,($\pm$0.54)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.98}}\scalebox{0.99}\,($\pm$0.49)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.72}}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.77}\scalebox{0.99}\,($\pm$0.65)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{-5.02}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}13.0\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Sim75}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.17}\scalebox{0.99}\,($\pm$0.76)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.53}}\scalebox{0.99}\,($\pm$0.73)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.55}\scalebox{0.99}\,($\pm$0.82)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.39}\scalebox{0.99}\,($\pm$0.78)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.86}\scalebox{0.99}\,($\pm$0.63)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{39.55}}\scalebox{0.99}\,($\pm$0.46)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{3.81}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{12.2}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}12.2\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{3.53}\scalebox{0.99}\,($\pm$0.27)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{3.26}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.88}\scalebox{0.99}\,($\pm$0.24)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{3.17}}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{3.16}}\scalebox{0.99}\,($\pm$0.31)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{3.42}\scalebox{0.99}\,($\pm$0.31)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{10.00}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}12.2\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Rec2}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{52.05}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{51.97}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{54.68}}\scalebox{0.99}\,($\pm$0.19)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{51.65}\scalebox{0.99}\,($\pm$0.06)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{53.52}\scalebox{0.99}\,($\pm$0.41)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{54.88}}\scalebox{0.99}\,($\pm$0.27)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{4.00}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{5.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.2\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.67}\scalebox{0.99}\,($\pm$2.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.40}\scalebox{0.99}\,($\pm$2.27)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{10.74}\scalebox{0.99}\,($\pm$1.76)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.81}\scalebox{0.99}\,($\pm$2.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{6.54}}\scalebox{0.99}\,($\pm$1.20)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{7.49}}\scalebox{0.99}\,($\pm$2.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{9.91}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.2\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Rec5}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 

& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{53.98}}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{53.45}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{53.45}\scalebox{0.99}\,($\pm$0.31)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{53.85}\scalebox{0.99}\,($\pm$0.18)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{52.80}\scalebox{0.99}\,($\pm$0.17)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{56.08}}\scalebox{0.99}\,($\pm$0.59)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{4.81}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{5.8}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.4\hspace{-0.01cm} }\end{tabular}
\\ 
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.49}}\scalebox{0.99}\,($\pm$0.68)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.03}}\scalebox{0.99}\,($\pm$0.67)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.41}\scalebox{0.99}\,($\pm$0.56)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.66}\scalebox{0.99}\,($\pm$0.68)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.27}\scalebox{0.99}\,($\pm$0.49)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.03}\scalebox{0.99}\,($\pm$0.47)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{2.75}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.4\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Rec10}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{52.20}\scalebox{0.99}\,($\pm$0.81)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{51.70}\scalebox{0.99}\,($\pm$0.44)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{52.34}}\scalebox{0.99}\,($\pm$0.35)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{50.80}\scalebox{0.99}\,($\pm$0.58)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{47.72}\scalebox{0.99}\,($\pm$0.20)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{54.22}}\scalebox{0.99}\,($\pm$0.52)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{6.41}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.6\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{6.2}}
\\ 
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.33}\scalebox{0.99}\,($\pm$0.37)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.25}\scalebox{0.99}\,($\pm$0.53)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.87}\scalebox{0.99}\,($\pm$0.43)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.07}\scalebox{0.99}\,($\pm$0.46)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.00}\scalebox{0.99}\,($\pm$0.52)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.32}\scalebox{0.99}\,($\pm$0.62)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{-8.00}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.6\hspace{-0.01cm} }\end{tabular}
\\ \midrule
\multirow{4}{*}{\hspace{-0.0cm}{\textbf{Abrupt}}\hspace{-0.01cm}} 
& \multirow{2}{*}{\makecell[c]{VTAB-19T}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{28.23}\scalebox{0.99}\,($\pm$0.14)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{28.11}\scalebox{0.99}\,($\pm$0.20)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{26.71}\scalebox{0.99}\,($\pm$0.29)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{28.48}\scalebox{0.99}\,($\pm$0.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{30.83}}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{32.39}}\scalebox{0.99}\,($\pm$0.32)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{13.76}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{18.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}18.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.15}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.43}\scalebox{0.99}\,($\pm$0.55)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{9.48}\scalebox{0.99}\,($\pm$0.54)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.50}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.01}}\scalebox{0.99}\,($\pm$0.23)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.30}}\scalebox{0.99}\,($\pm$0.69)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{31.90}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}18.0\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-5T}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{34.31}\scalebox{0.99}\,($\pm$0.04)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{34.03}\scalebox{0.99}\,($\pm$0.05)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{35.30}\scalebox{0.99}\,($\pm$0.41)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{34.17}\scalebox{0.99}\,($\pm$0.04)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.27}}\scalebox{0.99}\,($\pm$0.18)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{38.67}}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{9.81}}\%\hspace{-0.01cm} }\end{tabular}
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}5.0\end{tabular}}
& \multirow{2}{*}{\makecell[c]{5.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.55}\scalebox{0.99}\,($\pm$1.13)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.88}\scalebox{0.99}\,($\pm$1.09)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{17.72}\scalebox{0.99}\,($\pm$1.29)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.57}\scalebox{0.99}\,($\pm$1.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{12.84}}\scalebox{0.99}\,($\pm$0.98)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{13.25}}\scalebox{0.99}\,($\pm$1.00)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{14.58}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.0\hspace{-0.01cm} }\end{tabular}
\\
\bottomrule
\end{tabular}
}
\label{tbl:overall_perf}
% \vspace{-0.5cm}
\end{table*}


==> tables/overall_perf_unif_varying.tex <==
%\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \bgroup
\def\arraystretch{1.1}% make the row margin compact
\begin{table*}[t!]
\small
% \tiny
% \scriptsize
% \small
\centering
%\vspace*{-0.2cm}
\caption{Performance comparison of \algname{} against CL baselines using prompt tuning across uniformly and varying shift scenarios. This table shows the last accuracy as well as the average improvement and number of semantic groups by \algname{}; ``{\it Avg.~Improv.}'' denotes the average of the relative improvements over the best universal\,(LAE) and specific\,(S-Prompts) prompting methods. The best and second-best values are highlighted in bold and underlined, respectively.}
\vspace*{0.2cm}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
% {@{}c|c||C{1.85cm}c|C{1.85cm}c|C{1.85cm}cc@{}}
{@{}cc|c|ccccc|cccc@{}}
\toprule
\multirow{2}{*}{\hspace{-0.0cm}\makecell[c]{Shifting\\Scenarios}\hspace{-0.0cm}}&\multirow{2}{*}{\makecell[c]{CL\\Datasets}} &\multirow{2}{*}{\makecell[c]{Metrics}}
& \multicolumn{5}{c|}{{ {Prompt Tuning CL Algorithms}}} 
& \multicolumn{3}{c}{{ {\algname{} }}}\\%\cline{3-14} 

& & & \multicolumn{1}{c}{\hspace{-0.0cm}{L2P}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{VPT}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{LAE}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{DP}}
& \multicolumn{1}{c|}{\hspace{-0.01cm}{S-Prompts}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{\algname{}}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{\textit{Avg. Improv.}}}
& \multicolumn{1}{c}{\hspace{-0.01cm}{\textit{\#~Semantics}}}
\\ \midrule

% # Mild ###############################################################
\multirow{4}{*}{\hspace{-0.0cm}{\parbox{1.5cm}{\centering\textbf{Uniformly Mild}}}\hspace{-0.01cm}} 
& \multirow{2}{*}{\makecell[c]{ImageNet-R}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{68.05}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{69.31}\scalebox{0.99}\,($\pm$0.09)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{70.11}}\scalebox{0.99}\,($\pm$0.12)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{67.81}\scalebox{0.99}\,($\pm$0.19)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{65.89}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{69.45}}\scalebox{0.99}\,({$\pm$0.14})\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{2.13}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{1.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.17}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.27}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.05}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.99}}\scalebox{0.99}\,($\pm$0.18)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.71}\scalebox{0.99}\,($\pm$0.22)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.94}}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{28.2}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{CIFAR100}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{84.55}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{85.34}}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{85.16}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{84.79}\scalebox{0.99}\,($\pm$0.14)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{83.73}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{85.31}}\scalebox{0.99}\,($\pm$0.11)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{1.02}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{1.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{5.59}}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.19}\scalebox{0.99}\,($\pm$0.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.05}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{5.04}}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.41}\scalebox{0.99}\,($\pm$0.13)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.21}\scalebox{0.99}\,($\pm$0.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{0.32}}\%\hspace{-0.01cm} }\end{tabular}
% & \multirow{2}{*}{\makecell[c]{1.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}1.0\hspace{-0.01cm} }\end{tabular}
\\
\midrule
\multirow{4}{*}{\hspace{-0.0cm}{\parbox{1.5cm}{\centering\textbf{Uniformly Abrupt}}}\hspace{-0.01cm}} 
& \multirow{2}{*}{\makecell[c]{VTAB-19T}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{28.23}\scalebox{0.99}\,($\pm$0.14)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{28.11}\scalebox{0.99}\,($\pm$0.20)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{26.71}\scalebox{0.99}\,($\pm$0.29)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{28.48}\scalebox{0.99}\,($\pm$0.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{30.83}}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{32.39}}\scalebox{0.99}\,($\pm$0.32)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{12.58}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{18.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}18.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.15}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.43}\scalebox{0.99}\,($\pm$0.55)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{9.48}\scalebox{0.99}\,($\pm$0.54)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.50}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.01}}\scalebox{0.99}\,($\pm$0.23)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.30}}\scalebox{0.99}\,($\pm$0.69)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{36.25}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}18.0\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-5T}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{34.31}\scalebox{0.99}\,($\pm$0.04)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{34.03}\scalebox{0.99}\,($\pm$0.05)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{35.30}\scalebox{0.99}\,($\pm$0.41)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{34.17}\scalebox{0.99}\,($\pm$0.04)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.27}}\scalebox{0.99}\,($\pm$0.18)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{38.67}}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{5.12}}\%\hspace{-0.01cm} }\end{tabular}
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}5.0\end{tabular}}
& \multirow{2}{*}{\makecell[c]{5.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.55}\scalebox{0.99}\,($\pm$1.13)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.88}\scalebox{0.99}\,($\pm$1.09)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{17.72}\scalebox{0.99}\,($\pm$1.29)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{15.57}\scalebox{0.99}\,($\pm$1.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{12.84}}\scalebox{0.99}\,($\pm$0.98)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{13.25}}\scalebox{0.99}\,($\pm$1.00)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{13.29}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.0\hspace{-0.01cm} }\end{tabular}
\\ \midrule
\multirow{13}{*}{\hspace{-0.0cm}{\textbf{Varying}}\hspace{-0.01cm}} 
& \multirow{2}{*}{\makecell[c]{VTAB-Sim25}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.28}\scalebox{0.99}\,($\pm$0.50)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.24}\scalebox{0.99}\,($\pm$0.57)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.57}\scalebox{0.99}\,($\pm$0.72)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.72}\scalebox{0.99}\,($\pm$0.60)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.72}}\scalebox{0.99}\,($\pm$0.40)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{39.56}}\scalebox{0.99}\,($\pm$0.59)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{3.71}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{16.4}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}16.4\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{6.73}}\scalebox{0.99}\,($\pm$0.79)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.23}\scalebox{0.99}\,($\pm$0.65)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{9.51}\scalebox{0.99}\,($\pm$0.87)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{6.90}}\scalebox{0.99}\,($\pm$0.88)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.11}\scalebox{0.99}\,($\pm$0.53)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.10}\scalebox{0.99}\,($\pm$0.73)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{14.56}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}16.4\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Sim50}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.14}\scalebox{0.99}\,($\pm$0.36)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.30}\scalebox{0.99}\,($\pm$0.50)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.85}\scalebox{0.99}\,($\pm$0.73)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.22}\scalebox{0.99}\,($\pm$0.53)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.97}}\scalebox{0.99}\,($\pm$0.51)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{39.27}}\scalebox{0.99}\,($\pm$0.51)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{2.24}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{13.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}13.0\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.53}\scalebox{0.99}\,($\pm$0.71)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.22}\scalebox{0.99}\,($\pm$0.57)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.02}\scalebox{0.99}\,($\pm$0.54)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.98}}\scalebox{0.99}\,($\pm$0.49)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.72}}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.77}\scalebox{0.99}\,($\pm$0.65)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{1.70}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}13.0\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Sim75}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.17}\scalebox{0.99}\,($\pm$0.76)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{38.53}}\scalebox{0.99}\,($\pm$0.73)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.55}\scalebox{0.99}\,($\pm$0.82)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{38.39}\scalebox{0.99}\,($\pm$0.78)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{37.86}\scalebox{0.99}\,($\pm$0.63)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{39.55}}\scalebox{0.99}\,($\pm$0.46)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{4.89}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{12.2}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}12.2\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{3.53}\scalebox{0.99}\,($\pm$0.27)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{3.26}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.88}\scalebox{0.99}\,($\pm$0.24)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{3.17}}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{3.16}}\scalebox{0.99}\,($\pm$0.31)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{3.42}\scalebox{0.99}\,($\pm$0.31)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{24.34}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}12.2\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Rec2}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{52.05}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{51.97}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{54.68}}\scalebox{0.99}\,($\pm$0.19)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{51.65}\scalebox{0.99}\,($\pm$0.06)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{53.52}\scalebox{0.99}\,($\pm$0.41)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{54.88}}\scalebox{0.99}\,($\pm$0.27)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{1.44}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{5.0}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.2\hspace{-0.01cm} }\end{tabular}
\\
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.67}\scalebox{0.99}\,($\pm$2.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.40}\scalebox{0.99}\,($\pm$2.27)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{10.74}\scalebox{0.99}\,($\pm$1.76)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.81}\scalebox{0.99}\,($\pm$2.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{6.54}}\scalebox{0.99}\,($\pm$1.20)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{7.49}}\scalebox{0.99}\,($\pm$2.07)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{13.31}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.2\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Rec5}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 

& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{53.98}}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{53.45}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{53.45}\scalebox{0.99}\,($\pm$0.31)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{53.85}\scalebox{0.99}\,($\pm$0.18)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{52.80}\scalebox{0.99}\,($\pm$0.17)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{56.08}}\scalebox{0.99}\,($\pm$0.59)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{5.56}}\%\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{5.8}}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.4\hspace{-0.01cm} }\end{tabular}
\\ 
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{4.49}}\scalebox{0.99}\,($\pm$0.68)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{4.03}}\scalebox{0.99}\,($\pm$0.67)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.41}\scalebox{0.99}\,($\pm$0.56)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.66}\scalebox{0.99}\,($\pm$0.68)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.27}\scalebox{0.99}\,($\pm$0.49)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{5.03}\scalebox{0.99}\,($\pm$0.47)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{13.87}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.4\hspace{-0.01cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{2}{*}{\makecell[c]{VTAB-Rec10}}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$A_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{52.20}\scalebox{0.99}\,($\pm$0.81)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{51.70}\scalebox{0.99}\,($\pm$0.44)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\underline{52.34}}\scalebox{0.99}\,($\pm$0.35)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{50.80}\scalebox{0.99}\,($\pm$0.58)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{47.72}\scalebox{0.99}\,($\pm$0.20)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textbf{54.22}}\scalebox{0.99}\,($\pm$0.52)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{8.37}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.6\hspace{-0.01cm} }\end{tabular}
& \multirow{2}{*}{\makecell[c]{6.2}}
\\ 
& & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.01cm}\bm{$F_{last}$}\hspace{-0.01cm}}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{6.33}\scalebox{0.99}\,($\pm$0.37)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.25}\scalebox{0.99}\,($\pm$0.53)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{7.87}\scalebox{0.99}\,($\pm$0.43)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.07}\scalebox{0.99}\,($\pm$0.46)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.00}\scalebox{0.99}\,($\pm$0.52)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{8.32}\scalebox{0.99}\,($\pm$0.62)\hspace{-0.01cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}{\textit{-4.85}}\%\hspace{-0.01cm} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.01cm}5.6\hspace{-0.01cm} }\end{tabular}
\\
\bottomrule
\end{tabular}
}
\label{tbl:overall_perf}
\vspace{-0.5cm}
\end{table*}


==> tables/overall_perf_wFGT_unif_varying.tex <==
%\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \bgroup
\def\arraystretch{1.4}% make the row margin compact
\begin{table*}[t!]
\small
% \tiny
% \scriptsize
% \small
\centering
%\vspace*{-0.2cm}
\caption{
Performance comparison of \algname{} against CL baselines using prompt tuning across uniformly and varying shift scenarios. This table shows the forgetting as well as the average improvement and number of semantic groups by \algname{}; ``{\it Avg.~Improv.}'' denotes the average of the relative improvements over the best universal\,(LAE) and specific\,(S-Prompts) prompting methods.
% The best and second-best values are highlighted in bold and underlined, respectively.
}
\vspace*{0.2cm}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
% {@{}c|c||C{1.85cm}c|C{1.85cm}c|C{1.85cm}cc@{}}
{@{}cc|ccccc|ccc@{}}
\toprule
\multirow{2}{*}{\hspace{-0.0cm}\makecell[c]{Shifting\\Scenarios}\hspace{-0.0cm}}&\multirow{2}{*}{\makecell[c]{CL\\Datasets}} 
& \multicolumn{5}{c|}{{ {Prompt Tuning CL Algorithms}}} 
& \multicolumn{2}{c}{{ {\algname{} }}} \\ %\cline{3-14} 
& & \multicolumn{1}{c}{\hspace{-0.15cm}{L2P}\hspace{-0.15cm}}
& \multicolumn{1}{c}{\hspace{-0.15cm}{VPT}\hspace{-0.15cm}}
& \multicolumn{1}{c}{\hspace{-0.15cm}{LAE}\hspace{-0.15cm}}
& \multicolumn{1}{c}{\hspace{-0.15cm}{DP}\hspace{-0.15cm}}
& \multicolumn{1}{c|}{\hspace{-0.15cm}{S-Prompts}\hspace{-0.15cm}}
& \multicolumn{1}{c}{\hspace{-0.15cm}{\algname{}}\hspace{-0.15cm}}
& \multicolumn{1}{c}{\hspace{-0.15cm}{\textit{Avg. Improv.}}\hspace{-0.15cm}}
% & \multicolumn{1}{c}{\hspace{-0.15cm}{\textit{\#~Semantics}}}
\\ \midrule
\multirow{6}{*}{\hspace{-0.0cm}{\textbf{Varying}}\hspace{-0.15cm}} 
& \multirow{1}{*}{\makecell[c]{VTAB-Sim25}}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textbf{6.73}}\scalebox{0.99}\,($\pm$0.79)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{7.23}\scalebox{0.99}\,($\pm$0.65)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{9.51}\scalebox{0.99}\,($\pm$0.87)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\underline{6.90}}\scalebox{0.99}\,($\pm$0.88)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{7.11}\scalebox{0.99}\,($\pm$0.53)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{7.10}\scalebox{0.99}\,($\pm$0.73)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textit{14.56}}\%\hspace{-0.15cm} }\end{tabular}
\\ %\addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{1}{*}{\makecell[c]{VTAB-Sim50}}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{5.53}\scalebox{0.99}\,($\pm$0.71)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{5.22}\scalebox{0.99}\,($\pm$0.57)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{7.02}\scalebox{0.99}\,($\pm$0.54)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\underline{4.98}}\scalebox{0.99}\,($\pm$0.49)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textbf{4.72}}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{5.77}\scalebox{0.99}\,($\pm$0.65)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textit{1.70}}\%\hspace{-0.15cm} }\end{tabular}
\\ %\addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{1}{*}{\makecell[c]{VTAB-Sim75}}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{3.53}\scalebox{0.99}\,($\pm$0.27)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{3.26}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{5.88}\scalebox{0.99}\,($\pm$0.24)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\underline{3.17}}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textbf{3.16}}\scalebox{0.99}\,($\pm$0.31)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{3.42}\scalebox{0.99}\,($\pm$0.31)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textit{24.34}}\%\hspace{-0.15cm} }\end{tabular}
\\ \addlinespace[0.3ex]\cline{2-9}\addlinespace[0.5ex]
& \multirow{1}{*}{\makecell[c]{VTAB-Rec2}}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{7.67}\scalebox{0.99}\,($\pm$2.10)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{8.40}\scalebox{0.99}\,($\pm$2.27)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{10.74}\scalebox{0.99}\,($\pm$1.76)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{7.81}\scalebox{0.99}\,($\pm$2.07)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textbf{6.54}}\scalebox{0.99}\,($\pm$1.20)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\underline{7.49}}\scalebox{0.99}\,($\pm$2.07)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textit{13.31}}\%\hspace{-0.15cm} }\end{tabular}
\\ %\addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{1}{*}{\makecell[c]{VTAB-Rec5}}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\underline{4.49}}\scalebox{0.99}\,($\pm$0.68)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textbf{4.03}}\scalebox{0.99}\,($\pm$0.67)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{6.41}\scalebox{0.99}\,($\pm$0.56)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{5.66}\scalebox{0.99}\,($\pm$0.68)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{5.27}\scalebox{0.99}\,($\pm$0.49)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{5.03}\scalebox{0.99}\,($\pm$0.47)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textit{13.87}}\%\hspace{-0.15cm} }\end{tabular}
\\ %\addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{1}{*}{\makecell[c]{VTAB-Rec10}}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{6.33}\scalebox{0.99}\,($\pm$0.37)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{8.25}\scalebox{0.99}\,($\pm$0.53)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{7.87}\scalebox{0.99}\,($\pm$0.43)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{8.07}\scalebox{0.99}\,($\pm$0.46)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{8.00}\scalebox{0.99}\,($\pm$0.52)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{8.32}\scalebox{0.99}\,($\pm$0.62)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textit{-4.85}}\%\hspace{-0.15cm} }\end{tabular}
\\ \midrule
% # Mild ###############################################################
\multirow{2}{*}{\hspace{-0.0cm}{\parbox{1.5cm}{\centering\textbf{Uniformly Mild}}}\hspace{-0.15cm}} 
& \multirow{1}{*}{\makecell[c]{ImageNet-R}}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{5.17}\scalebox{0.99}\,($\pm$0.10)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{5.27}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{6.05}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\underline{4.99}}\scalebox{0.99}\,($\pm$0.18)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{7.71}\scalebox{0.99}\,($\pm$0.22)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textbf{4.94}}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textit{28.2}}\%\hspace{-0.15cm} }\end{tabular}
\\ %\addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{1}{*}{\makecell[c]{CIFAR100}}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\underline{5.59}}\scalebox{0.99}\,($\pm$0.08)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{6.19}\scalebox{0.99}\,($\pm$0.07)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{6.05}\scalebox{0.99}\,($\pm$0.21)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textbf{5.04}}\scalebox{0.99}\,($\pm$0.15)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{6.41}\scalebox{0.99}\,($\pm$0.13)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{6.21}\scalebox{0.99}\,($\pm$0.07)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textit{0.32}}\%\hspace{-0.15cm} }\end{tabular}
\\ \midrule
\multirow{2}{*}{\hspace{-0.0cm}{\parbox{1.5cm}{\centering\textbf{Uniformly Abrupt}}}\hspace{-0.15cm}} 
& \multirow{1}{*}{\makecell[c]{VTAB-19T}}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{6.15}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{6.43}\scalebox{0.99}\,($\pm$0.55)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{9.48}\scalebox{0.99}\,($\pm$0.54)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{5.50}\scalebox{0.99}\,($\pm$0.42)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textbf{4.01}}\scalebox{0.99}\,($\pm$0.23)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\underline{4.30}}\scalebox{0.99}\,($\pm$0.69)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textit{36.25}}\%\hspace{-0.15cm} }\end{tabular}
\\ %\addlinespace[0.3ex]\cdashline{2-11}\addlinespace[0.5ex]
& \multirow{1}{*}{\makecell[c]{VTAB-5T}}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{15.55}\scalebox{0.99}\,($\pm$1.13)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{15.88}\scalebox{0.99}\,($\pm$1.09)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{17.72}\scalebox{0.99}\,($\pm$1.29)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{15.57}\scalebox{0.99}\,($\pm$1.07)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textbf{12.84}}\scalebox{0.99}\,($\pm$0.98)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\underline{13.25}}\scalebox{0.99}\,($\pm$1.00)\hspace{-0.15cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.15cm}{\textit{13.29}}\%\hspace{-0.15cm} }\end{tabular}
\\ \bottomrule
\end{tabular}
}
\label{tbl:overall_fgt}
% \vspace{-0.5cm}
\end{table*}


==> x-deleted.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

% \noindent\textbf{Continual Learning.}
\subsection{Continual Learning}
%In continual learning, we encounter a sequence of tasks $D = \{D_1, \dots, D_T\}$, with $T$ denoting the total number of encountering tasks. Task $t$ has a data stream $D_t = \{(x^i_t, y^i_t)\}_{i=1}^{m_t}$ derived from a joint distribution over input space $\mathcal{X}_t$ and one-hot encoded label space $\mathcal{Y}t$, with $m_t$ being the number of instances for that task. The goal in continual learning is to formulate a classifier that maximizes test accuracy for all encountered tasks $\{1, 2, \dots, T\}$, with restricted access to the data streams $D_{t^{\prime}}$ of prior tasks where $t^\prime < t$. In realistic CL scenarios, these data streams may exhibit diverse environments and varying inter-task similarities, serving as a comprehensive testbed for evaluating the adaptability of continual learning approaches.

In CL, we consider a sequence of tasks $\mathcal{T}=\langle \tau_1, \cdots, \tau_{|\mathcal{T}|} \rangle$ for a data stream $\mathcal{D} = \langle D_{1}, \cdots, D_{|\mathcal{T}|}\rangle$, where each sub-dataset $D_{t} = \{(x_t, y_t)\}$ for the $t$-th task is derived from a joint distribution of an input space $\mathcal{X}_{t}$ and a label space $\mathcal{Y}_{t}$. The goal in CL is to continuously learn a classifier that maximizes test accuracy for all encountered tasks $\{\tau_1,\tau_2,\cdots,\tau_t\}$, without having access to data streams $D_{t^\prime<t}$ of prior tasks. In realistic settings, these data streams may come from diverse environments, and thus associated tasks exhibit varying inter-task similarities, calling for adaptable CL approaches.
% $\{1, 2, \dots, t\}$

\smallskip
% \noindent\textbf{Prompt Tuning Continual Learning.}
\subsection{Prompt-based Continual Learning}
%Current prompt-based continual learning methods\,\cite{l2p, dp, lae} mostly employ a pretrained backbones like ViT, which is primarily composed of $L$ transformer blocks. Each of these blocks utilizes a multi-head attention module to extract pertinent features. Then, prompts, small additional weight parameters, are prepended as additional input for the transformer block's attention module. Recently, as discussed in \cite{DP, LAE}, prompts primarily serve as a prefix, prepending exclusively to the keys and values of the input. A single prompt ${\rm P} \in \mathbb{R}^{p \times d}$ is defined as a sequence of tokens, each with $d$ dimensions, and the sequence has a length of $p$. This prompt is compatible with key and value configurations in various prompt-based CL techniques. 
%
%
% In the context of our study, let ${\rm {E}}_l \in \mathbb{R}^{n \times d}$ denote the input tokens, introduced to the $l$-th transformer block. Then, the attention mechanism can then be reformulated as:
% \begin{equation}
% \begin{gathered}
% {\rm {E}}^\prime_{l} = {\rm Attention}({\rm {Q}}, {\rm {K^\prime}}, {\rm {V^\prime}}) ~\text{where}~ \\
% {\rm {Q}} = {\rm {E}}_l{\rm W}^Q,~{\rm {K^\prime}} = [{\rm P}; {\rm {E}}_l{\rm W}^K],~{\rm {V^\prime}} = [{\rm P}; {\rm {E}}_l{\rm W}^V].
% \end{gathered}
% \label{eq:attn_prompts}
% \end{equation}
% Here, ${\rm W}^Q$, ${\rm W}^K$, and ${\rm W}^V$ denote the linear projection matrices for the query, key, and value input tokens, in that order. The symbol $[\cdot;\cdot]$ represents concatenation, and a single-head attention mechanism is defined as
% % ${\rm W}^Q$, ${\rm W}^K$, and ${\rm W}^V$ are linear projections matrices for query, key, and value tokens, respectively; $[\cdot;\cdot]$ is concatenation; and the attention mechanism is defined as: 
% \begin{equation}
% {\rm Attention}({\rm {Q}}, {\rm {K}}, {\rm {V}})=\rm{softmax}\left(\frac{{\rm Q}{\rm K}^T}{\sqrt{d}}\right){\rm V}
% \label{eq:attn}
% \end{equation}
%
Recent prompt-based CL methods\,\cite{wang2022dualprompt, wang2022learning, gao2023unified} mostly employ a pretrained backbone (e.g., ViT\,\cite{dosovitskiy2021an}) with $L$ transformer blocks, where each of these blocks utilizes a multi-head attention module to extract pertinent features. A prompt, in this setting, refers to a set of vectors that provide auxiliary context or guide the attention mechanism towards specific patterns in the data for a task:
\begin{equation}
{\rm P} = [{\rm \mathbf{p}}_1,\dots, {\rm \mathbf{p}}_p ] \in \mathbb{R}^{p \times d}
\label{eq:prompt}
\end{equation}
where $p$ and $d$ are the number and the dimensionality of tokens ${\rm \mathbf{p}}_i$, respectively. The prompt serves as a prefix to the input for the transformer block's attention module, being prepended exclusively to the keys and values\,\cite{wang2022dualprompt, gao2023unified}.
% Specifically, given input tokens ${\rm {E}}_l \in \mathbb{R}^{n \times d}$ at an $l$-th transformer block, a prompt ${\rm P}$ is incorporated as follows to produce output tokens ${\rm {E}}^\prime_{l}$:
% \begin{equation}
% \begin{gathered}
% {\rm {E}}^\prime_{l} = {\rm Attention}({\rm {Q}}, {\rm {K^\prime}}, {\rm {V^\prime}}) ~\text{where}~ \\
% {\rm {Q}} = {\rm {E}}_l{\rm W}^Q,~{\rm {K^\prime}} = [{\rm P}; {\rm {E}}_l{\rm W}^K],~{\rm {V^\prime}} = [{\rm P}; {\rm {E}}_l{\rm W}^V],
% \end{gathered}
% \label{eq:attn_prompts}
% \end{equation}
% where ${\rm W}^Q$, ${\rm W}^K$, and ${\rm W}^V$ respectively denote the linear projection matrices for the input tokens to query $Q$, key $K$, and value $V$. Here, $[\cdot;\cdot]$ represents concatenation, and a single-head attention is defined as ${\rm Attention}({\rm {Q}}, {\rm {K}}, {\rm {V}})=\rm{softmax}\left(\frac{{\rm Q}{\rm K}^T}{\sqrt{d}}\right){\rm V}$.
% \begin{equation}
% {\rm Attention}({\rm {Q}}, {\rm {K}}, {\rm {V}})=\rm{softmax}\left(\frac{{\rm Q}{\rm K}^T}{\sqrt{d}}\right){\rm V}.
% \label{eq:attn}
% \end{equation}
%
%In this framework, while the pre-trained backbone remains fixed, the prompts are the main elements subjected to learning. Consequently, these prompts influence the output embeddings of the ViT’s transformer layers by permeating to the image patch tokens through attention mechanisms, thereby adapting to the specific task at hand.
%
% While the pre-trained backbone remains unchanged, the prepended prompts are optimized while attending to the input tokens, thereby adapting to specific tasks at hand.

\smallskip
\noindent \textbf{Prompt Tuning and Inference.}
Universal and specific strategies are used for managing and selecting prompts. 
First, \emph{universal} prompting employs a constant prompt ${\rm P}$ on all tasks. The optimization objective for a given task $\tau_t$ with $D_t$ is to minimize the cross-entropy loss $\ell_{ce}$:
\begin{equation}
\small
\min_{{\rm P}, {\rm k}, \phi} \ell_{ce} (f_\phi(f([x_t; {\rm P}])), y_t), 
\label{eq:objective}
\end{equation}
where $f_\phi$ is a classifier, and $f$ is a pre-trained model that receives the concatenation of the input tokens $x_t$ and the prompt ${\rm P}$ and then returns the $[\mathtt{CLS}]$ token for prediction.
%
Second, \emph{specific} prompting employs a collection of task-specific prompts $\{{\rm P}_t \mid \tau_t\in\mathcal{T} \}$ and corresponding learnable prompt keys $\{{\rm k}_t \mid \tau_t\in\mathcal{T} \}$ to determine the prompt to be used. The optimization objective is to maximize the similarity between the input and the prompt key, in addition to minimizing the cross-entropy loss:
\begin{equation}
\small
\min_{{\rm P}_t, {\rm k}_t, \phi} \ell_{ce} (f_\phi(f([x_t; {\rm P}_t])), y_t) - \lambda{\rm d}(f(x_t),{\rm k}_t),
\label{eq:spcf_objective}
\end{equation}
where $\lambda$ is a balancing coefficient and $\rm{d}(\cdot)$ is a similarity function (e.g., cosine similarity).
%between the [$\mathtt{CLS}$] token of an input $x$ by the pre-trained model and the key ${\rm k}_t$

During inference, given a testing instance $x$, the matching prompt $P_{\hat{t}}$ is chosen to maximize the similarity between $f(x_t)$ and its prompt key ${\rm k}_{t}$:
\begin{equation}
\hat{t} = \arg\max_{t} {\rm d}(f(x_t), {\rm k}_{t}).
\label{eq:preliminary-inference}
\end{equation}

%\section{Proposed Method: \algname{}}
%\section{Semantic-aware Adaptive Prompting}
\section{Adaptive Prompting via Semantic Grouping}

\label{sec:methodology}

% \input{figures/algorithm}


% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=0.98\textwidth, ]{figures/model_arch.pdf}
%     % \includegraphics[width=0.95\textwidth, ]{figures/model_arch.pdf}
%     \caption{\textbf{Detailed view of the main components of \algname{}}:
%     }
%     \label{fig:model_arch}
%     % \vspace*{-0.6cm}
% \end{figure*}

\subsection{Problem Formulation}
\label{subsec:problem}

% optimal grouping -> computationally prohibitive \\
% objective: group semantically tasks \\
% CL: online assignment function \\
% task order dependency->pronounced in "relevant" tasks \\
% two-level: 1) group relevant 2) refine relevant

% 교수님: 아래 내용은 intro에서 말해두고 여기서는 생략
% Given the computational impracticality of identifying optimal task groups, \algname{}, inspired by MTL\,\cite{1,2,3}, finds semantically similar tasks for the maximization of positive transfer.

% 교수님: 아래 내용은 이따가 정의할 때 쓰고 여기서는 생략
 % ; for instance, Figure \ref{fig:model_arch}(a) indicates that Task 3 and 4 classify images within the realms of architectural and satellite semantics, respectively.
 % $E=\{e_1, \dots,e_T\}$, with each semantic encapsulating the abstract concept of a task.

\begin{comment}
% For future reivision: JGL
\end{comment}

The \emph{adaptive} prompting problem is in between the two extremes---universal and specific prompting. That is, at the $t$-th task, while universal and specific prompting strategies maintain \emph{one} and $t$ prompts, respectively, our adaptive prompting strategy manages \emph{from one to $t$} prompts depending on the semantic shifts observed so far. Thus, the key challenge is to lie in the management of the best collection of prompts, which is realized by our novel \emph{semantic grouping} process. 

We formalize the adaptive prompting problem through a \emph{semantic grouping} of CL tasks, such that it can capture generalizable knowledge in a group with similar tasks while avoiding catastrophic forgetting from different groups with dissimilar tasks.
Specifically, for a sequence of tasks $\mathcal{T}=\langle \tau_1, ... \tau_{t} \rangle$, we aim to find task semantic groups $\mathcal{G}=\{G_1,\dots, G_{|\mathcal{G}|}\}$ by minimizing
\begin{equation}
J(\mathcal{G}) =  \sum_{G \in \mathcal{G}} \sum_{\tau_i, \tau_j \in G} {\rm d}\big( {\rm s}(\tau_i), {\rm s}(\tau_j)\big) + \alpha|\mathcal{G}|,
\label{eq:obj}
\end{equation}
where $G$ is a group of tasks, ${\rm s}(\tau)$ is a semantic representation of a task $\tau$ which can be derived by a task-specific prompt ${\rm P}_\tau$\footnote{Task-specific prompts are known to capture the intrinsic patterns of task data distributions. See Definition \ref{def:task_semantic_embedding} for details.}, ${\rm d}(\cdot)$ is the distance among semantic representations, and the term $\alpha|\mathcal{G}|$ penalizes trivial solutions such as overgrouping.
After finding semantic groups, we can assign a group prompt ${\rm P}_G$ for each semantic group $G$ to maximize positive transfer among semantically similar tasks.

\begin{comment}
We formalize the adaptive prompting problem in CL through semantic grouping of tasks.
Specifically, for a sequence of tasks $\mathcal{U}=\langle t_1, ... t_{|\mathcal{U}|} \rangle$, we aim to find semantic groups $\mathcal{G}=\{G_1,\dots, G_{|\mathcal{G}|}\}$, where $G_i$ is a semantic group of tasks and has a corresponding prompt $P_i$ 

the semantic representation of a task $t_i$ is denoted as ${\rm s}(t_i)$, encapsulating the abstract concept of the task.
These groups are designed to maximize the total intra-group similarity, thereby facilitating maximal positive transfer among tasks when training a prompt for each group. Formally, we aim to obtain the optimal semantic group $\mathcal{G}^*$ by minimizing 
\begin{equation}
J(\mathcal{G}) =  \sum_{i=1}^{|\mathcal{G}|} \sum_{t_1, t_2 \in G_i} {\rm d}\big( {\rm s}(t_1), {\rm s}(t_2)\big) + \alpha|\mathcal{G}|
\label{eq:obj}
\end{equation}
where ${\rm d}(\cdot)$ denotes internal semantic distance and the term $\alpha|G|$ penalizes trivial solutions such as overgrouping.
\end{comment}

However, finding semantic groups by Eq.\,\eqref{eq:obj} to obtain the group prompts is infeasible in CL environments since only the current dataset $D_{t}$ is accessible, so we can not retune the group prompts from the past datasets.
%Thus, in CL, the semantic grouping should be solved in an \emph{online} manner, such that the group prompts of the past tasks are fixed and the semantic grouping of the current task is performed on top of the past groups.
A trivial solution is an online greedy approach; the current task is assigned to a past group if they are close in semantic representation or otherwise create a new semantic group. This approach often falls into the local optima as the greedy group assignment is \emph{irreversible} thereby accumulating substantial noises in grouping (see Section \ref{subsec:analysis_of_semantic_refinement} for further analysis).
Therefore, this calls for a novel adaptive prompting scheme to ensure more accurate semantic group assignments.



\begin{comment}
However, optimization for future unknown tasks and past tasks is not feasible in CL due to the sequential arrival of tasks. Therefore, a greedy approximation solution is employed by utilizing a grouping function $F$, which updates the grouping state $\mathcal{G}^{{i}}$ at task $t_i$ with a new task semantic ${\rm s}(t_i)$. In updating, $F$ decides whether to integrate the new task into an existing semantic group or to create a new group, based on a predefined distance threshold $\tau$.
Then, the state of grouping at $t_{i+1}$, denoted as $\mathcal{G}^{{{i+1}}}$, is defined by $\mathcal{G}^{{i+1}}=F_{i+1}(\mathcal{G}^{{i}};\tau) $. 
With each decision, the function aims to minimize $J(\mathcal{G}^{{i}})$, so that $J(\mathcal{G}^{{i+1}}) \leq J(\mathcal{G}^{{i}})$ to maintain or improve the intra-group similarity.


This greedy approach, while practical, does not guarantee the global optimization of $J(\mathcal{G})$. The initial decision made for task $t_i$ may not remain optimal with the inclusion of subsequent tasks at task $t_j$ where $i<j$. This is because tasks near the semantic group boundaries might be better suited to different groups as more tasks are introduced. Moreover, the decisions are irreversible, meaning that once a task is assigned to a group, it cannot be reassigned, even if later tasks indicate a more suitable grouping. This limitation impedes the effectiveness of prompt learning by restricting positive transfer. 

% This greedy approach, while practical, does not guarantee the global optimization of $J(\mathcal{G})$ since it makes \textit{irreversible} decisions based on partial information. In retrospect, the greedy decision may become suboptimal as more tasks become accessible. Specifically, suboptimal grouping mainly occurs in tasks whose semantic representations are situated in close proximity to the \textit{boundary(?)} of semantic groups. As CL progresses, their optimal group membership of such tasks can be easily shifted to the more suited semantic group, although irreversible. Inaccurate semantic groups directly make the learning of prompts ineffective by impeding positive transfer.

% This function optimizes semantic groups $\mathcal{G}^{{i}}$ for each task $t_i$. Specifically, when a new task ${t_{i+1}}$ arrives, $F$ updates the previous semantic groups $\mathcal{G}^{{i}}$ based on the new task semantics ${\rm s}(t_{i+1})$. 
% $F$ decides whether to integrate the new task into an existing semantic group or to create a new group, based on a predefined distance threshold $\tau$ as $\mathcal{G}^{{i+1}} = F_{t_{i+1}}^\tau(\mathcal{G}^{{i}})$.
% Formally, the optimization of semantic groups for each new task arrival is formalized as:
% \begin{equation}
% \mathcal{G}^{t_{i+1}} = F(\mathcal{G}^{t_{i}}, {\rm s}({t_{i+1}}); \tau) \text{ such that } J(\mathcal{G}^{t_{i+1}}) \leq J(\mathcal{G}^{t_{i}}).
% \label{eq:online-func}
% \end{equation}
% $F^\tau_{t_{i+1}}(\mathcal{G}^{{i}})$
\end{comment}

\subsection{Overview of \algname{}}
\label{subsec:overview}

% we propose \algname{} for \textit{refinable} semantic grouping that facilitates the restoration of optimal groupings and prompts in light of new tasks. 
%\algname{} achieves this through a two-level semantic grouping process.

We propose \algname{} that performs adaptive prompting via two-phase semantic grouping; (1) \emph{macroscopic semantic assignment} and (2) \emph{microscopic semantic refinement}.
In the macroscopic semantic assignment, \algname{} assigns the current task to a semantic super-group encompassing broader semantic space which provides refinable slacks to reconcile past groupings. Then, in the microscopic semantic refinement, \algname{} adjusts the semantic groups to restore optimal groupings, ensuring that the prompts are prepared based on the precise semantic groups. {\red{The overall procedures are illustrated in Figure \ref{x} and Algorithm \ref{x}.}}
 

% To precisely refine semantic groups $\mathcal{G}^{{i}}$ for each task $t_i$, \algname{} employs \textit{two-level semantic grouping}. 
% Initially, \algname{} establishes \textit{macroscopic} semantic groups that have broad coverage to accommodate boundary tasks and facilitate future refinements\,(Section \ref{subsec:mac}). 
% Then, \algname{} re-evaluates optimal groupings within the \textit{macroscopic} semantic groups as tasks arrive and corrects previous suboptimal grouping by refining {macroscopic} semantic groups into \textit{microscopic} semantic groups, thereby forming the $\mathcal{G}^{{t}}$\,(Section \ref{subsec:mic}). 

% The presence of inaccurate semantic groups directly leads to the learning inefficiency of prompts by preventing positive transfer.
% Thus, we propose \algname{} that 
% To address this in an efficient and accurate way, \algname{} first selects \textit{macroscopic} semantic groups to encompass boundary tasks and allow future refinements on such tasks as CL progresses. Then, through a re-evaluation of the evolving task relationships, \algname{} dynamically refines \textit{macroscopic} semantic groups into more precise, microscopic semantic groups. 



% Given their potential for inaccurate grouping, these \textit{boundary(?)} tasks are prime candidates for re-evaluation as more tasks arrive and the semantic landscape of the CL system evolves. 

% \smallskip
% \begin{theorem}
% % Assume that a subset $\mathcal{S}\in\tilde{\mathcal{D}}$ follows $\alpha_\mathcal{S}$-expansion and $\beta_\mathcal{S}$-separation, where $\alpha_\mathcal{S} \le \alpha$. Then, the training error of a Re-labeling model $\theta_{\mathcal{S}}$ trained on $\mathcal{S}$ is bounded by the inverse of the total reduced neighborhood confidence $\sum_{x\in{\tilde{\mathcal{D}}}} C_{\mathcal{N}}(x;\mathcal{S})$ such that,

% % Given a dataset \(D\) and an online assignment algorithm \(F : \mathcal{P}(D) \rightarrow S\), where \(\mathcal{P}(D)\) is the power set of \(D\) and \(S\) the set of all possible clusterings of \(D\). Let \(A \subseteq D\) be a subset with intra-cluster distances less than \(\epsilon\) and \(B \subseteq D\) a subset with inter-cluster distances more than \(\epsilon\), where \(d\) is a metric on \(D\) and \(\epsilon\) a small positive real number. If \(C\) is order-sensitive, then the probability of a change in clustering outcome due to input permutation is higher for \(A\) than for \(B\), formally expressed as:

% % Given a set of task \(U\) and an online assignment algorithm $F$, let \(A \subseteq U\) be a subset with intra-group distances less than \(\epsilon\) and \(B \subseteq U\) a subset with inter-group distances more than \(\epsilon\), where \(\epsilon\) a small positive real number. If \(C\) is order-sensitive, then the probability of a change in clustering outcome due to input permutation is higher for \(A\) than for \(B\), formally expressed as:
% % \[ P(\Delta_F(A)) > P(\Delta_F(B)) \]
% \begin{equation}
% \begin{gathered}
% P(\Delta_C(A)) > P(\Delta_C(B))
% % {Err}(\theta_{\mathcal{S}}) \le {{2 \cdot |\mathcal{S}| \cdot {Err}(\theta_{\mathcal{M}}) }\over \sum_{x\in{\tilde{\mathcal{D}}}} {C_\mathcal{N}(x;\mathcal{S})} } + {2 \cdot \alpha_{\mathcal{S}}\over {\alpha}_{\mathcal{S}}-1}\cdot{\beta_{\mathcal{S}}},
% \end{gathered}
% \label{eq:error_bound}
% \end{equation}
% % where $\theta_{\mathcal{M}}$ is a model trained with the supervised loss in Eq.~\eqref{eq:relabeling} on a given clean set $\mathcal{M}\subset \mathcal{S}$.
% \label{theorem:neighbor_confidence_to_label_correction}
% \begin{proof}
% % tbd
% % We extend the label denoising theorem in \,\cite{wei2020theoretical} by incorporating the influence of the subset to the expansion factor $\alpha_\mathcal{S}$.
% % The complete proof is available in Appendix \ref{appendix:proof_theory3.3}. 
% \end{proof}
% \end{theorem}


% Therefore, to address this effectively, we propose OURS, which initially selects relevant tasks and subsequently performs refinement for these relevant tasks.

% solving this optimization is infeasible in CL due to the \textit{inaccessibility} of previous or upcoming tasks. Instead, the nature of CL, with tasks arriving \textit{sequentially}, necessitates the online updates of these semantic groups for every task. Formally, the semantic groups at task $t+1$ are updated as
% \begin{equation}
% G^{t+1}=F(G^{t}, e_{t+1})) \text{~such that~} J(G^{t+1})\geq J(G^{t})
% % G^{t+1}=F(\{e_i\}_{i=1}^t, {\rm order}(\{e_i\}_{i=1}^t)) \text{~such that~} J(G^{t+1})\geq J(G^{t})
% \label{eq:online-func}
% \end{equation}
% where $F$ is an online assignment function that modifies the semantic grouping $G^t$ based on the new semantics $e_{t+1}$.

% Unfortunately, due to its sequential nature, the online assignment function $F$ has an inherent dependency on task order where the same set of tasks arriving in a different order can result in different outcomes of semantic grouping, indicating a certain task order can lead to inaccurate grouping different to the optimal grouping. Importantly, such dependency leads to more frequent inaccurate assignments among \textit{relevant} tasks than largely distinct tasks as in Theorem \ref{}.

% Therefore, to address this effectively, we propose OURS, which initially selects relevant tasks and subsequently performs refinement for these relevant tasks.


% % aim
% \algname{} realizes adaptive prompt management for CL tasks through \textit{semantic}-aware adaptation. The key strategy is to universally learn tasks with relevant semantics while specifically targeting tasks that present novel semantics. Following this, tasks are learned using prompts that correspond to the carefully determined semantics. The overall procedure is depicted in Figure \ref{fig:model_arch} and outlined in Algorithm \ref{alg:overall}.



% Central to \algname{} is the concept of \textit{semantics}, which pertains to the intrinsic patterns insights tied to a task's data distribution. For instance, Figure \ref{fig:model_arch}(a) indicates that Task 3 and 4 classify images within the realms of architectural and satellite semantics, respectively. To capture this, we define the notion of a \textit{task semantic embedding}---a vector representation that encapsulates the core essence of a task---in Definition \ref{def:task_semantic_embedding}. This vector is derived using a prompt from Eq.~\eqref{eq:prompt} over a warm-up training period. 
% \begin{definition}{\sc (Task Semantic Embedding)}.
% Given warm-up prompt \( {\rm P}^w_t \) for task \( t \), the \textit{task semantic embedding} is computed as
% \begin{equation}
% e_t = {\rm Normalize}\left({\rm AvgPool}({\rm P}^w_t)\right) \in \mathbb{R}^{d},
% \label{eq:task_semantic_embedding}
% \end{equation}
% where {\rm AvgPool($\cdot$)} is a function that aggregates the outputs across all $p$ lengths, encapsulating the semantics for task $t$ and {\rm Normalize($\cdot$)} performs $l_2$-normalization.
% \label{def:task_semantic_embedding}
% \end{definition}

% Building on this, the objective of \algname{} is to find the particular partitioning\,(clustering) of CL tasks into semantic groups that maximize the total intra-cluster similarity, leading to the maximal positive transfer. Such a cluster is termed a \textit{semantic group}, outlined as: 
% \begin{definition}{\sc (Semantic Group)}.
% The \textit{semantic group} for a semantic $s$ is represented as 
% \begin{equation}
% G_s = \{ t~ |~ \psi(t)=s, ~ t\in \{1,\dots,T\}\},
% \label{eq:task_semantic_group}
% \end{equation}
% where $\psi(t)$ returns an assigned semantic for a given task $t$.
% \label{def:task_semantic_group}
% \end{definition}
% \noindent 
% % This semantic group can be as few as one when all tasks share similar semantics or as many as $t$ for completely distinct tasks. 
% Formally, we aim to find optimal semantic grouping $G^*$ such that
% \begin{equation}
% G^* = \underset{{G}}{\mathrm{argmax}} \left( \sum_{i=1}^{|G|} \sum_{t_1, t_2 \in G_i} {\rm Similarity}(e_{t_1}, e_{t_2}) \right)
% \label{eq:obj}
% \end{equation}
% where ${G}$ is the set of semantic groups defined as ${G}=\{ G_1, \dots, G_{|G|} \}$, and ${\rm Similarity}(e_{t_1}, e_{t_2})$ denotes the similarity between task semantic embeddings $e_{t_1}$ and $ e_{t_2}$. 

% % Furthermore, in CL, the diverse and sequential nature of tasks often gives rise to order sensitivity.
% Solving this optimization problem directly is computationally infeasible due to its combinatorial nature and the inherent inaccessibility of CL to previous or upcoming tasks.
% Furthermore, in CL, as tasks are processed sequentially without a global view of entire tasks, such a short-sighted, or greedy, assignment approach often causes incorrect semantic grouping. Though reassignment of processed tasks can rectify these errors, it is computationally inefficient if applied indiscriminately.

% To achieve both precision in semantic grouping and computational efficiency, \algname{} introduces a \textit{two-level hierarchical semantic grouping}, drawing inspiration from the pre-clustering algorithm\,\cite{canopy}. Initially, we aim to identify \textit{macroscopic semantic groups} that grasp global semantics of CL tasks\,(Section \ref{subsec:mac}). Subsequently, we refine these groups to determine the final \textit{semantic groups} as per Definition \ref{def:task_semantic_group}\,(Section \ref{subsec:mic}). 

% Finally, these semantic groups form the basic elements for training prompts and subsequent inferences\,(Section \ref{subsec:tr_inf}). As tasks undergo refinement from non-universal to universal, there arises a potential mismatch where prompts aligned with these tasks may remain unprocessed. To maintain the adaptability of the refinement, we identify candidate sub-semantic groups that, while currently designated as non-universal, show strong potential for merging in the future. \algname{} proactively pre-tunes and reserves prompts for these candidate groups.

% \input{figures/algorithm}

\subsection{Phase 1: Macroscopic Semantic Assignment}
\label{subsec:mac}
% 1. 목표 설명: capture coarse semantic groups to accommodate potential refinements in the context of CL where complete knowledge of future tasks is not available.
% 1-1 Advantages of Macroscopic Grouping: providing a broad overview & accommodation for future refinements (this approach sets the stage for more detailed, microscopic groupings in subsequent phases.)
% 2. Definition of the macroscopic semantic group
% 3. task semantic explanation + definition
% 4. application of Greedy Approximation
% 5. Reiterate the use of the greedy approximation approach as tasks arrive
% 6. 

% Without complete knowledge of future tasks, a sequential grouping of similar tasks may result in suboptimal grouping.
To allow potential refinements in semantic grouping, we form a set ${\mathcal{S}}^{t}=\{S^t_1, \cdots, S^t_{|{\mathcal{S}}^{t}|}\}$ of \emph{semantic super-groups}. 
%Specifically, for each new task, we assign the task to an existing {macroscopic} semantic group or create a new {macroscopic} semantic group. %after extracting the task semantic representation, 

\begin{definition}{\sc (Semantic Super Group)}
\label{def:macro_semantic_group}
A \textit{semantic super-group} $S^{t}$ given all seen tasks $\mathcal{T}^t=\langle \tau_1, \cdots, \tau_t \rangle$ is a set of tasks that are within $R$ from the centroid of the super-group in the semantic representation space. Formally,
\begin{equation}
S^{ t} = \{\tau \in \mathcal{T}^t~|~ {\rm d}(\tau, S^t) \leq R \},
\label{eq:macro_semantic_group}
\end{equation}
where ${\rm d}(\tau, S^t)$ is the distance between the task semantic $s(\tau)$ and the group centroid ${1 \over |S^t|}\sum_{\tau \in S^t} {\rm s}(\tau)$\,\cite{zhang1996birch}.
\end{definition}

\begin{comment}
\begin{definition}{\sc (Macroscopic Semantic Group)}
Let $\tau_1$ denote the distance threshold indicating a highly divergent semantic difference. The \textit{macroscopic semantic group} for a macro-level semantic $m$ at task $t_i$ comprises a collection of tasks that maintain an internal distance smaller than the threshold, $\tau_1$. That is,
\begin{equation}
{M}_m^{i} = \{t~|~ {\rm d}({M}_m^{i}) \leq \tau_1 \},
\label{eq:macro_semantic_group}
\end{equation}
where \({\rm d}({M}_m^{i})\) computes the internal semantic distance as $\left( \frac{1}{|{M}_m^{i}|} \sum_{t s\in {M}_m^{i}} \left( {\rm s}(t) - {\rm Centroid}({M}_m^{i}) \right)^2 \right)^{1/2}$ and ${\rm Centroid}({M}_m^{i}) = \frac{1}{|{M}_m^{i}|}\sum_{t \in {M}_m^{i}} {\rm s}(t)$.
\label{def:macro_semantic_group}
\end{definition}
\end{comment}

\smallskip
\noindent\textbf{Task Semantic Extraction.} 
%To perform semantic super grouping, it is essential to extract the \textit{semantic representation} ${\rm s}(\tau)$ of each task.
%%, which pertains to the intrinsic patterns of a task's data distribution. 
%For instance, Figure \ref{fig:overview}(a) indicates that Task A classify images within the realms of staples semantic, respectively. 
%Thus, we define a \textit{task semantic representation} in Definition \ref{def:task_semantic_embedding}, derived from a task-specific prompt efficiently obtained after a short period of training, called a warm-up period. 
Given a new task $\tau^t$, we allow a warm-up training period to get a very initial prompt $P_{\tau}$ through the objective goal in Equation 
\ref{eq:spcf_objective}. Then, a task semantic representation is extracted as follows.

\begin{definition}{\sc (Task Semantic Representation)}.
Given a warm-up prompt \( {\rm P}_{\tau} \) for a task \( \tau \), the \textit{task semantic representation} ${\rm s}(\tau)$ is computed as
\begin{equation}
{\rm s}(\tau) = {\rm Normalize}\left({\rm AvgPool}({\rm P}^w_{\tau})\right) \in \mathbb{R}^{d},
\label{eq:task_semantic_embedding}
\end{equation}
where {\rm AvgPool($\cdot$)} pools the prompt averaged over all $p$ tokens and {\rm Normalize($\cdot$)} performs $l_2$-normalization.
\label{def:task_semantic_embedding}
\end{definition}



% Initially, \algname{} captures global semantics in the CL distribution via \textit{macroscopic semantic groups}, in Definition \ref{def:macro_semantic_group}. Simultaneously, these semantic groups allow opportunities for future refinements for the final semantic grouping.

% \begin{definition}{\sc (Macroscopic Semantic Group)}
% Let $\tau_1$ denote the distance threshold indicating highly divergent semantic difference. The \textit{macroscopic semantic group} for a macro-level semantic $m$ comprises a collection of tasks that maintain an internal distance smaller than the threshold, $\tau_1$. That is,
% \begin{equation}
% \mathcal{G}_m = \{t~|~ {\rm Avg\text{-}Dist}(\mathcal{G}_m) \leq \tau_1 \},
% \label{eq:macro_semantic_group}
% \end{equation}
% where \({\rm Avg\text{-}Dist}(\mathcal{G}_m)\) computes the internal distance to its centroid as $\left( \frac{1}{|\mathcal{G}_m|} \sum_{t \in \mathcal{G}_m} \left( e_t - {\rm Centroid}(\mathcal{G}_m) \right)^2 \right)^{1/2}$ and ${\rm Centroid}(\mathcal{G}_m) = \frac{1}{|\mathcal{G}_m|}\sum_{t \in \mathcal{G}_m} e_t$.

% \label{def:macro_semantic_group}
% \end{definition}



\noindent\textbf{Macroscopic Assignment.} 
Given the previous semantic super-groups $\mathcal{S}^{t-1}$ and the current task $\tau_t$, we obtain new super-groups $\mathcal{S}^t$ by using an assignment function $\mathcal{A}_R$ with a threshold $R$, i.e,  $\mathcal{S}^t=\mathcal{A}_R(\tau_t; \mathcal{S}^{t-1})$. 
If the current task $\tau_t$ is semantically irrelevant to \emph{any} of the previous super-groups $\mathcal{S}^{t-1}$, a novel semantic super-group of the task $\tau_t$ is initialized; otherwise, it is assigned to the closest semantic super-group. Formally, $\mathcal{A}_R(\tau_t; \mathcal{S}^{t-1})$ is defined as
\begin{equation}
\small
\begin{aligned}
&\begin{cases}
\mathcal{S}^{t-1} \cup \{ \tau_t \} &\text{if } ~~ {\rm d}(\tau_t, S) > R \quad \forall S\in\mathcal{S}^{t-1} \\
\mathcal{S}^{t-1}\backslash S^{t-1}_* \cup \{ S^{t-1}_* \cup \{ \tau_t \} \} &\text{if } ~~ {\rm d}(\tau_t, S_*^{t-1}) \leq R,
\end{cases}
\label{eq:mac_assign}
\end{aligned}
\end{equation}
where $S_*^{t-1}=\arg\max_{S^{t-1} \in \mathcal{S}^{t-1}}d(\tau_t,S^{t-1})$.
%is the closest semantic super-group in $\mathcal{S}^{t-1}$ to the current task $\tau_t$.

%With the obtained super-groups $\mathcal{S}^t$, we can perform semantic refinement to find accurate semantic groups for prompting.

\smallskip
\noindent\textbf{Preparatory Semantic Groups Collection.} 
We refine semantic super-groups into finer \emph{semantic groups} (see Definition \ref{def:microscopic semantic groups}) that better generalize to the underlying task semantics with a \emph{single} prompt. It also requires readily preparing prompts dedicated to each refined semantic group even without accessing the past tasks. To this end, we additionally manage a collection of \emph{preparatory semantic groups} (see Definition \ref{def:Preparatory groups}) to ensure that each preparatory semantic group has the prompt adapted to all tasks it contains, facilitating on-the-fly prompt-tuning in an online manner. %Additionally, we investigate the consequences of merging prompts post hoc without adaptation to the refined groups in Section \ref{subsec:anal_micro_refine}.


\begin{definition}{\sc (Semantic Groups)}.
Given a {semantic super-group} ${S}^t$, a set ${\mathcal{G}}^{S^t}$ of \textit{semantic groups} $G^{S^t}$  further divides the super-group with finer granularities.
\begin{equation}
\small
\begin{gathered}
\mathcal{G}^{S^t} = \{ G^{S^t}_{1}, \cdots, G^{S^t}_{|\mathcal{G}^{S^t}|} \} \quad\text{s.t.} \quad S^t = \bigcup_{j=1}^{|\mathcal{G}^{S^t}|} G^i_{j},
%\forall i ~~ {\rm d}(\tau, G^{S^t}_i) \leq r
%
\end{gathered}
\label{eq:microscopic semantic groups}
\end{equation}
%where $G^{S^t}_{i}$ is the $i$-th semantic group of the super-group $S^t$.
\label{def:microscopic semantic groups}
\end{definition}


\begin{definition}{\sc (Preparatory Semantic Groups)}.
Given a {semantic super-group} ${S^t}$, a set ${\mathcal{P}}^{S^t}$ of \textit{preparatory semantic groups} is the candidate set of possible semantic groups, accumulated over past tasks, such as
\begin{equation}
\small
\begin{gathered}
%\mathcal{P}^{S^t} = \{ \hat{\mathcal{G}^{S^t}_{1}}, \cdots, \hat{\mathcal{G}^{S^t}_{c}} \} \cup \mathcal{P}^{S^{t-1}},
\mathcal{P}^{S^t} = \hat{\mathcal{G}^{S^t}} \cup \mathcal{P}^{S^{t-1}},
\end{gathered}
\label{eq:Preparatory groups}
\end{equation}
where $\hat{\mathcal{G}^{S^t}}$ is determined by the k-means algorithm\,\cite{bradley1998refining} over ${S^t}$ based on semantic similarities.  
\label{def:Preparatory groups}
\end{definition}

Note that the number of clusters can be decided by a widely-used distribution indicator (e.g., silhouette score\,\cite{rousseeuw1987silhouettes}). Each semantic group $G^{S^t} \in \hat{\mathcal{G}^{S^t}}$ is equipped with the prompt that has been trained over past tasks and/or adapted to the new task $\tau_t$ if $\tau_t \in G^{S^t}$. It is also possible to add multiple $\hat{\mathcal{G}^{S^t}}$ with different numbers of clusters prioritized by the distribution indicator. 

\begin{comment}
as:
\begin{equation}
\small
\hat{\mathcal{G}^{S^t}} = \{ \hat{G}^{S^t}_{1}, \dots, \hat{G}^{S^t}_{k} \} = {\rm K\text{-}means}({S^t}; k).
% C^{j}({M}_m^{t}) = {\rm K\text{-}means}({M}_m^{t}; c^*),
\label{eq:candidate_sets}
\end{equation}
\end{comment}

\begin{comment}
Given the task semantic representation ${\rm s}(t)$, we apply the greedy grouping functions $F$ with the threshold $R$ as \(M^{i}=F_{i}(M^{i-1};\tau_1)\) where $M^i=\{M_1^i,\dots,M_{|M|}^i\}$ is a set of macroscopic semantic groups for at task $t_i$. This assigns the new task to the existing macroscopic semantic groups or creates a new group based on the \textit{semantic distance} between the new task and the existing macroscopic semantic groups. 


% Upon the arrival of a new task, as illustrated in Figure \ref{fig:model_arch}(a), \algname{} performs a \textit{sequential clustering} with $\tau_1$, \(\rm Seq{\text -}cluster_{\tau_1}(\cdot)\). This involves estimating the \textit{semantic distance} between the new task and the existing macroscopic semantic groups, followed by assigning the new task to the most appropriate group. 

% \smallskip
% \noindent\textbf{Semantic Distance Estimation.} 
\textit{Semantic distance} is measured as the internal distance within a new task's semantic representation and those of the closest semantic group\,\cite{zhang1996birch}, as formulated in Definition \ref{def:task_semantic_distance}.
\begin{definition}{\sc (Semantic Distance)}.
Given the macroscopic semantic group $M^{i-1}$, and the semantic representation ${\rm s}(t_i)$, the \textit{semantic distance} is
\begin{equation}
\small
\begin{gathered}
d_{i} = {\rm d}\left({M}_{m^*}^{i-1} \cup \{t_i\}\right), \\
\text{~where~} m^* = \arg\min_{m} {\rm ED}\left( {\rm Centroid}\left(\mathcal{M}_m^{i-1}\right), {\rm s}(t) \right),\\
\end{gathered}
\label{eq:task_semantic_distance}
\end{equation}
and \({\rm ED}(\cdot,\cdot)\) computes the Euclidean distance.
\label{def:task_semantic_distance}
\end{definition}



%
Then, for a task with semantic distance $d_{i}$, (i) a task with a large distance\,($d_{i} > \tau_1$) is directed to a newly-initialized macroscopic semantic group due to its \textit{novel semantic}; (ii) a task with relevant semantic distance\,($d_{i} \leq \tau_1$) is allocated to an existing macroscopic semantic group due to its \textit{relevant semantic}. The assigned macroscopic semantic group is updated as:
\begin{equation}
\small
% \mathcal{G}(t) \leftarrow{}
\begin{cases}
% \mathcal{M}_{|{M}|+1}^{i+1} = \{t\} & \text{if } d_{i+1} > \tau_1 \quad \text{(i) Novel Semantic,} \\
\text{A new group } \{t_i\} & \text{if } d_{i} > \tau_1 \quad \text{(i) Novel Semantic,} \\
{M}_{m^*}^i \cup \{t_i\} & \text{if } d_{i} \leq \tau_1 \quad \text{(ii) Relevant Semantic.}
\end{cases}
\label{eq:mac_assign}
\end{equation}
The closest semantic index $m^*$ is derived from Eq.~\eqref{eq:task_semantic_distance}. 
% Here, $\mathcal{G}(t)$ denotes the macroscopic semantic group allocated to task $t$. 
\end{comment}

% Refining these semantic groups can be effective but computationally expensive if applied indiscriminately. Thus, we propose an assignment approach reminiscent of the pre-clustering algorithm\,\cite{canopy} where our goal is to first identify \textit{macroscopic semantic groups} and subsequently concentrate refinement efforts on tasks with marginal differences, ensuring both computational efficiency and precision in task groupings.
% Specifically, as a result of the assignment, (i) a task with clearly large distance is directed to a newly-initialized semantic group to \textit{specifically} tune on a novel task; (ii) a task with neutral semantic distance is allocated to an existing semantic group, which is \textit{remergable} by further refinement.

% The overall task assignment is controlled by two distance thresholds, $\tau_1$ and $\tau_2$, with $\tau_1 > \tau_2$. 
% While $\tau_1$ acts as a preliminary mechanism for clustering tasks with significantly distinct semantics, $\tau_2$ ultimately determines if a task aligns universally or specifically with existing semantics.
% Thus, for a task with semantic distance $d_t$, the macroscopic semantic group is determined by $\tau_1$,
% \begin{equation}
% G(t) \leftarrow{}
% \begin{cases}
% G_{|G|+1} = \{e_t\} & \text{if } d_t > \tau_1 \quad (\text{Specific}) \\
% G_{s^*} \cup \{e_t\} & \text{if } d_t \leq \tau_1 \quad (\text{Remergable})
% \end{cases}
% \end{equation}
% Here, $G(t)$  denotes the macroscopic semantic group allocated to task $t$. The closest semantic index $s^*$ is derived from Eq.~\eqref{eq:task_semantic_distance}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%TODO%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Phase 2: Microscopic Semantic Refinement}  
\label{subsec:mic}

\algname{} further refines the semantic super-group $S^t$ of the new task $\tau_t$ to restore more generalizable semantic groups and their prompts from the preparatory groups $\mathcal{P}^{S^t}$.
% Then, in both cases, the new task $\tau_t$ is assigned to the refined or unchanged semantic groups, i.e., $\{ \tau_t \}$ or $\{ G^{S^t}_* \cup \{ \tau_t \}\}$.   

% To determine whether refinement is necessary, we focus on whether the addition of $\tau_t$ to sematic super-group $S^{t-1}$ can derive a more generalizable semantic group than previous semantic groups of $S^{t-1}$.


% We refine semantic super-groups into \emph{semantic groups} that better generalize to the underlying task semantics. 
% Also, to train prompts of the refined semantic groups without accessing the past task datasets, we further manage a set of \emph{preparatory groups} for each super-group that ensures prompt-tuning in an online manner.


\begin{comment}
To restore optimal groupings by aligning with the evolved semantic context, we 
refine a macroscopic semantic group into a set of semantic groups\,(See Definition \ref{def:microscopic semantic groups}) that better generalize the updated semantics. Once refined, we obtain prompts for the semantic groups from an auxiliary repository of semantic groups and associated prompts, termed \textit{preparatory groups}, which does not require revisiting past tasks.

\begin{definition}{\sc (Semantic Groups)}.
Given a {semantic super-group} ${S}$ and a small grouping threshold $r$, the \textit{semantic groups} ${\mathcal{G}}^S$ of ${S}$ are
\begin{equation}
\small
\begin{gathered}
\mathcal{G}^S = \{ G^{S}_{1}, \cdots, G^S_{|\mathcal{G}^S|} \} \quad\text{s.t.}\quad\forall i ~~ {\rm d}(\tau, G^S_i) \leq r,
%{M}_m^{i} = \bigcup_{j=1}^{r_m} G^i_{(m,j)},
\end{gathered}
\label{eq:microscopic semantic groups}
\end{equation}
where $G^S_{i}$ is the $i$-th semantic group of the super-group $S$.
\label{def:microscopic semantic groups}
\end{definition}

\begin{definition}{\sc (Preparatory Groups)}.
Given a {semantic super-group} ${S}$, the \textit{preparatory groups} ${\mathcal{P}}^S$ are the candidate set of possible semantic groups such as
\begin{equation}
\small
\begin{gathered}
\mathcal{P}^S = \{ \hat{\mathcal{G}^{S}_{1}}, \cdots, \hat{\mathcal{G}^S_{c}} \},
%{M}_m^{i} = \bigcup_{j=1}^{r_m} G^i_{(m,j)},
\end{gathered}
\label{eq:microscopic semantic groups}
\end{equation}
where $c$ is the number of candidates. We find 
\label{def:microscopic semantic groups}
\end{definition}

\end{comment}



% \smallskip
% \noindent\textbf{Microscopic Refinement.} 
% We only refine a \emph{single} semantic super-group $S_{\text{refine}}$, i.e., $\{ \tau_t \}$ or $\{ S^{t-1}_* \cup \{ \tau_t \}\}$, that is changed in super-grouping at task $t$, ensuring an efficient refinement process.


\smallskip
\noindent\textbf{Refinement Criterion.} Intuitively, we examine the contribution of the new task to the reduction of semantic groups. When assuming each semantic group has the same coverage (i.e., the radius of $\gamma$R where $0<\gamma<1$), a set of fewer semantic groups better generalizes the underlying semantic contexts. That is, the goal of refinement for $S^t$ is to achieve $|\mathcal{G}^{S^t}|\leq|\mathcal{G}^{S^{t-1}}|$.

Specifically, we investigate various grouping options to alleviate the biased grouping, which is highly influenced by the order of tasks\,\cite{bradley1998refining, zhang1996birch}.
Inspired by simulation-based clustering\,\cite{celebi2013comparative, bradley1998refining}, we permutate task orders and execute grouping to identify the one with the fewest semantic groups. 

%The refinement process begins by permuting the original task order within the semantic super-group $S^t$ to generate a set of $\kappa$ virtual orders $\Bar{S}^t$. We then evaluate these permutations to find the task order $\hat{S}^{t}$ that results in the fewest semantic groups using the greedy assignment function $\mathcal{A}_r$ with radius $r$, computed as:
\begin{equation}
\hat{S}^{t} = \arg\min_{\hat{S}^{t}}|\mathcal{H}_{\gamma R}(\hat{S}^{t} \big)|,
\label{eq:min_group}
\end{equation}
where $\mathcal{H}_{\gamma R}({S}^t)$ is the recursive assignment $\mathcal{A}_{\gamma R}$ of the arbitrarily ordered tasks in $S^t$, i.e.,  $\mathcal{H}_{\gamma R}({S}^t) = \mathcal{A}_{\gamma R}(\tau_t, \mathcal{H}_r(S^{t-1}))$. 
%where $\mathcal{H}_r({S}^t)$ denotes the iterative application of $\mathcal{A}_r$ in a recursive manner as $\mathcal{A}_r(\tau_t, \mathcal{H}_r(S^{t-1}))$. 

%Consequently, if $|\mathcal{H}_r(\hat{S}^{t})|<|\mathcal{H}_r(\hat{S}^{t-1})|$, the semantic groups are updated to the refined groups. 
% , and ${\rm Count}(\cdot)$ calculates the number of generated semantic groups

\smallskip
\noindent\textbf{Semantic Groups Update.}
%As a result of refinement, the semantic groups are set to the grouping of $\hat{S}^{t}$ in Eq.~\eqref{eq:min_group}, i.e., $\mathcal{G}^{S^t}=\mathcal{H}(\hat{S}^{t})$. 
If $|\mathcal{H}_{\gamma R}(\hat{S}^{t})|<|\mathcal{G}^{S^{t-1}}|$, the semantic groups are updated, i.e., $\mathcal{G}^{S^t}=\mathcal{H}_{\gamma R}(\hat{S}^{t})$. Otherwise, previous semantic groups are kept and the new task is assigned to an existing semantic group or creates a new semantic group, i.e., $\mathcal{G}^{S^t}=\mathcal{A}_{\gamma R}(\tau_t, \mathcal{G}^{S^{t-1}})$. 
Note that once the new semantic groups are updated, their corresponding prompts can be retrieved from the ones equipped in the preparatory semantic groups $\mathcal{P}^{S^t}$ either directly or indirectly by further adapting to the current task $\tau_t$.


%appended to the preparatory groups ${\mathcal{P}}^{S^t}$ as they can also be replaced and restored throughout the refinement process.

% Suboptimal grouping is mainly due to the sequential nature of CL where the presentation order of early tasks biases overall groupings, as the early tasks influence the grouping of later ones\,\cite{bradley1998refining, zhang1996birch}. Thus, we implement a simulation-based refinement strategy, inspired by \cite{celebi2013comparative,
% bradley1998refining}, which executes grouping over various virtual task orders and identifies the optimal microscopic semantic grouping as per Eq.~\eqref{eq:microscopic semantic groups} that represents all tasks with the minimum number of groups.  


% \smallskip
% \noindent\textbf{Semantic Groups Formation.} %$\mathcal{G}^i$
% The semantic groups, $\mathcal{G}^t$, are the aggregate of refined microscopic semantic groups from all macroscopic semantic groups., as:
% \begin{equation}
% \mathcal{G}^t=\bigcup_{m=1}^{|M^t|} S(M^t_m).
% \label{eq:final_semantic_groups}
% \end{equation}
% Here, the unchanged macroscopic semantic groups in  Eq.~\eqref{eq:mac_assign} retain their previous microscopic semantic groups, i.e., $S({M}_m^{t})=S({M}_m^{t-1})$, and if the macroscopic semantic group already meets the threshold criterion, i.e., \({\rm d}({M}_m^{t}) \leq \tau_2\), it maintains itself as a microscopic semantic group, i.e., $S({M}_m^{t})={M}_m^{t}$.

% \smallskip
% \noindent\textbf{Preparatory Groups.}
% When semantic groups are refined, there must exist their corresponding prompts.
% Particularly, as past task data is inaccessible to tune the prompts in CL, \algname{} maintains \textit{preparatory groups} to proactively train prompts for potential semantic groupings. 
% Since tasks with close semantics are likely to be grouped, we create candidate sets of semantic groups, denoted as $C({M}_m^{t})$, through grouping tasks based on their semantic similarities. This process employs clustering algorithms like ${\rm K\text{-}means}$. The number of clusters is pre-determined by a widely-used distribution indicator, e.g., silhouette score\,\cite{rousseeuw1987silhouettes}. Formally, the $j$-th candidate set is defined as:
% \begin{equation}
% \small
% C^{j}({M}_m^{t}) = \{ G^t_{(m,1)}, \dots, G^t_{(m,c^*)} \} = {\rm K\text{-}means}({M}_m^{t}; c^*),
% % C^{j}({M}_m^{t}) = {\rm K\text{-}means}({M}_m^{t}; c^*),
% \label{eq:candidate_sets}
% \end{equation}
% where $c^*$ is the determined cluster number by the silhouette score.
% We also investigate the consequences of merging prompts post hoc without adaptation to prior tasks in Section \ref{subsec:anal_micro_refine}.


% Thus, without relying on the distance threshold, multiple candidate sets of semantic groups, $C(\mathcal{G}_m)$, are selected through a conventional clustering algorithm, where the cluster count is pre-determined by a distribution indicator, e.g., silhouette score\,\cite{rousseeuw1987silhouettes}. Formally, a single candidate set is obtained by:
% \begin{equation}
% C^{i}(\mathcal{G}_m) = {\rm K\text{-}means}_{c^*}(\mathcal{G}_m),
% \label{eq:candidate_sets}
% \end{equation}
% where $c^*$ is the determined cluster number by the silhouette score.
% We also investigate the consequences of post-merging without adaptation to prior tasks, such as by averaging the prompts' parameters in Section \ref{subsec:anal_micro_refine}.

% \big((F_{\Bar{t}_{n}} \circ \cdots \circ F_{\Bar{t}_1})(G_0; \tau_2) \big)


% suboptimal groupings might not have occurred if the tasks had been presented in a different order which enables new optimal semantic grouping. Thus, we employ a simulation-based refinement strategy that simulates various virtual task sequences to explore different grouping possibilities. By doing so, it aims to discover more optimal groupings that may not have been apparent in the original sequential task presentation.

% We initialize the parameters of a semantic group $G^i_j$ with the pre-tuned those of the group $G^i_j\setminus\{t\}$ and fine-tune them on the current task. For tasks introducing a novel semantic, the parameters are trained from scratch. 
\subsection{Prompt Tuning and Inference}  
\label{subsec:tr_inf}

\smallskip
\noindent\textbf{Overall Optimization.}
In the meanwhile, \algname{} proactively trains the prompts and the corresponding prompt keys for semantic groups in preparatory groups $\mathcal{P}^{S^t}$ to facilitate future semantic group refinements.
Let $\theta_t$ be a set of prompt-key pairs for the target semantic groups $\hat{G}^{S^t}$ in $\mathcal{P}^{S^t}$ containing a new task $\tau_t$, such as
\begin{equation}
    \theta_{t} = \{ ({\rm P}_{\hat{G}^{S^t}}, {\rm k}_{\hat{G}^{S^t}}) \mid \tau_t \in \hat{G}^{S^t} \in \mathcal{G}^{S^t} \in \mathcal{P}^{S^t} \}.
\label{eq:prompts4tuning}
\end{equation}
%\theta_{t} = \{ ({\rm P}_{\hat{G}^{S^t}}, {\rm k}_{\hat{G}^{S^t}}) \mid \tau_t \in \hat{G}^{S^t} ,\hat{G}^{S^t} \in \mathcal{G}^{S^t}, \mathcal{G}^{S^t} \in \mathcal{P}^{S^t} \}

Then, the optimization objective of \algname{} is to optimize the general across multiple prompts and keys for the target semantic groups:
\begin{equation}
\small
\min_{\theta_{t}, \phi} \mathbb{E}_{({\rm P}, {\rm k})\sim \text{U}(\theta_t)}\!\left[ \ell_{ce} (f_\phi(f([x_{t}; {\rm P}])),\! y_{t})\! - \!\lambda{\rm Sim}(f(x_{t}),\!{\rm k}) \right]\!, 
% \min_{({\rm P}, {\rm k})\sim \theta_{t}, \phi} \ell_{ce} (f_\phi(f([x_{t}; {\rm P}])[\mathtt{CLS}]), y_{t}) - \lambda{\rm Cosine}(q(x_{t}),{\rm k}), 
\label{eq:objective}
\end{equation}
where $({\rm P}, {\rm k})$ is uniformly sampled from $\theta_{t}$.
% where $f_{\rm P}$ transforms the input tokens using prompts as Eq.~\eqref{eq:attn_prompts}, and then forwards them to the pre-trained backbone, and $f_\phi$ is the classifier utilizing the [$\mathtt{CLS}$] token for prediction; $\rm{Cosine}(\cdot)$ denotes the cosine similarity function and $q(x)$ is the feature vector of the [$\mathtt{CLS}$] token from the pre-trained backbone. $\ell_{ce}$ and $\lambda$ denote the cross-entropy loss and a balancing coefficient between two loss terms, respectively.

\smallskip
\noindent\textbf{Semantic Group Inference.} During inference with semantic prompts, it is necessary to infer a semantic group for each testing instance. At task $\tau_t$, the semantic groups $\mathcal{G}^t$ are composed of the union of groups from all semantic super-groups, as:
\begin{equation}
\small
\mathcal{G}^t=\bigcup_{i=1}^{|\mathcal{S}^t|} \mathcal{G}^{S^t_i}.
\label{eq:final_semantic_groups}
\end{equation} 
For a test instance $x$, the identity of the inferred semantic group is determined by the query-key matching mechanism (Eq.~\eqref{eq:preliminary-inference}). Specifically, the group is identified as the $\hat{j}$-th semantic group within the $\hat{i}$-th semantic super-group, which is obtained as:
\begin{equation}
\hat{i},\hat{j} = \arg\max_{i,j} {\rm Sim}(q(x), {\rm k}_{G^{S_i^t}_{j}}).
\label{eq:inference}
\end{equation}

% $\hat{i}$,$\hat{j}$ is determined by:
% \begin{equation}
% \hat{i},\hat{j} = \arg\max_{i,j} {\rm Cosine}(q(x), {\rm k}_{G^{S_i^t}_{j}}).
% \label{eq:inference}
% \end{equation}


% Consequently, the semantic groups $\mathcal{G}^i$ at task $t_i$ are the aggregate of refined microscopic semantic groups from all macroscopic semantic groups, as:
% \begin{equation}
% \mathcal{G}^i=\bigcup_{m=1}^{|M^i|} S(M^i_m).
% \label{eq:final_semantic_groups}
% \end{equation}
% Here, if the macroscopic semantic group already meets the threshold criterion, i.e., \({\rm d}({M}_m^{t}) \leq \tau_2\), it maintains itself as a microscopic semantic group, i.e., $S({M}_m^{t})={M}_m^{t}$.

% \smallskip
% \noindent\textbf{Semantic Group Inference.} As the task identity prediction mechanism in \cite{wang2022learning, wang2022dualprompt}, each microscopic semantic group $G^i_j$ is inferred through the matching of the keys, which are optimized by Eq.~\eqref{eq:objective}. Given a test instance $x$, its semantic group identity is determined by:
% \begin{equation}
% \hat{i}, \hat{j} = \arg\max_{i,j} {\rm Cosine}(q(x), {\rm k}^i_j).
% \label{eq:inference}
% \end{equation}
% where $\rm{Cosine}(\cdot)$ denotes the cosine similarity function and $q(x)$ represents the feature vector tied to the [$\mathtt{CLS}$] token from our pre-trained architecture.


% for intermediate tasks
% This can make the quality of assignments susceptible to task order, especially with tasks having intermediate distances, leading to over-grouping where the number of identified semantic groups exceeds the ideal as described in Figure \ref{fig:order-sensitivity}. Such order-dependency, a known challenge in traditional clustering algorithms,\cite{kmeans, etc.}, is even more pronounced in online clustering. 
% Although tasks with clearly large or small distances provide groupings consistent with global clustering, those with intermediate distances are often sensitive to task order as described in Figure \ref{fig:order-sensitivity}.
% as in Figure {}: 예를 들어, Figure {}(a)의 예시에서 originally 3개의 task의 순서에 따라서 resulting number of groups가 달라짐

% for intermediate tasks
% Specifically, as a result of the assignment, i) a task with clearly large or small distance is directed to a newly-initialized semantic group to \textit{specifically} tune on a novel task or an existing semantic group, \textit{universally} tuned on previous similar tasks; ii) a task with intermediate semantic distance is allocated to a \textit{remergable} semantic group.
% As tasks progress, enriching our perspective on the CL environment, we perform a reassessment of the remergable group. This identifies tasks poised for universal applicability, amplifying overall generalizability.

% \min_{\theta_t, \phi} \ell_{ce} (f_\phi(f_{\theta_t}(x_t)), y_t) - \lambda {\rm Cosine}(q(x_t),\theta_t) 
% \min_{({\rm P}, {\rm k})\in\theta(t), \phi} \ell_{ce} (f_\phi(f_{P}(x_t)), y_t) - \gamma {\rm Cosine}() 
% OURS는 current task를 포함하는 sub-semantic groups에 대응되는 prompt parameters을 학습함.
% 이 prompts들은 하나씩 골라져서 Eq.(1)처럼 input tokens에 prepend되어 pre-trained model을 통과하게 됨.

% 이 prompt parmeters는 those corresponding to sub-semantic groups-{current_task}에서 copied and finetuned됨, additional knowledge being integrated without erasing the prior one.
% on the other hand, if no other elements in sub-semantic groups due to distinct semantics, prompt parameters are fully trained from scratch

% Overall, \algname minimizes the following loss function:
% train both prompts, keys, classification head 
% where classifer-head $f_\phi$, $f_p(t)$ the pre-trained architecture with prompts $p(t)$, l_ce, gamma. 
%  S(Gs) C(Gs)

% these sets of sub-semantic groups에서 

%  to implementation details?
% In terms of prompt tuning, novel semantic groups, which lack any relevant semantics, are fully trained from scratch while fine-tuning is adopted for existing semantics, ensuring that additional knowledge is integrated without erasing the prior one. 



% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=0.98\textwidth]{figures/model_arch.pdf}
%     % \caption{\textbf{ING}}
%     \vspace*{-0.3cm}
%     \caption{\textbf{Detailed view of the main components of \algname{}}: (a) drops the highly-activated features on the fused feature map according to the intensity $\kappa$; as in the example of the drop mask, the fusion facilitates identifying the background shortcuts from the signal of the high-level features on important parts such as the body of the dog. (b) adjusts the drop intensity $\kappa$ for the use in attentive debiasing. 
%     }
%     \label{fig:model_arch}
%     \vspace*{-0.2cm}
% \end{figure*}
% % Specifically, the coarse discriminative signals of the deep features pointing to a shortcut can be overlaid with essential parts, which should not be dropped.

% \noindent\textbf{Online Continual Learning.}
% We consider the online continual learning setting, where a sequence of tasks continually emerges with a set of new classes. Each data instance can be accessed only once unless it is stored in episodic memory. For the $t$-th task, let $D_t=\{(x^i_t,y^i_t)\}_{i=1}^{m_t}$ be a data stream obtained from a joint data distribution over $\mathcal{X}_t \times \mathcal{Y}_t$, where $\mathcal{X}_t$ is the input space, $\mathcal{Y}_t$ is the label space in a one-hot fashion, and $m_t$ is the number of instances of the $t$-th task. The goal of OCL is to train a classifier, such that it maximizes the test accuracy of all seen tasks $T=\{1,2, \dots, t\}$ at time $t$, with limited or no access to the data stream $D_{t^{\prime}}$ of previous tasks $t^{\prime}<t$.

% \medskip
% \noindent\textbf{Shortcut and Non-shortcut Features.}
% Let a DNN model trained on $(x,y) \sim \mathcal{X}\times\mathcal{Y}$ comprises a general feature extractor $f^{\theta}:\mathcal{X}\rightarrow\mathcal{Z}\in\mathbb{R}^d$ and a final classifier layer $g^{\text{w}}:\mathcal{Z}\rightarrow \mathbb{R}^{k}$, which is the multiplication of a linear weight matrix $\text{w}\in\mathbb{R}^{k\times d}$ and a feature $z\in \mathcal{Z}$ such that $g^{\text{w}}(z)=w\cdot z$. Here, $k$ is the number of classes, and $d$ is the dimensionality of a feature $z$. Let a \emph{feature} be the function mapping from the input space $\mathcal{X}$ to a real number; formally speaking, for the $i$-th sub-feature extractor of $f^{\theta}$ where $i\!\in\!\{1,2,\!\ldots\!,d\}$, $f^{\theta}_i:\mathcal{X}\rightarrow\mathbb{R}$. DNNs are known to have simplicity bias toward shortcut features which can easily distinguish between given classes\,\cite{geirhos2018imagenet, shah2020pitfalls, pezeshki2021gradient}. Then, the \emph{shortcut} and \emph{non-shortcut} features are defined by Definitions \ref{def:shortcut_feature} and \ref{def:non_shortcut_feature}, respectively.

% \begin{definition}{\sc (Shortcut Feature)}.
% Let $x$ and $\tilde{x}$ be the instances from seen and unseen data distributions $\mathcal{X}$ and $\mathcal{\tilde{X}}$, respectively, where $\mathcal{X}\cap\mathcal{\tilde{X}}=\emptyset$. We call a feature a \emph{shortcut} if it is not only highly activated ($\geq \rho$) for the seen data instance but also undesirably activated ($\geq \epsilon$) for the unseen data instance in expectation. That is,
% \vspace{-0.05cm}
% \begin{equation}
% f^{\theta}_{s}(\rho, \epsilon) : \mathbb{E}_{x \sim \mathcal{X}} \big[|f^{\theta}_s(x)| \big] \geq \rho ~\land ~ \mathbb{E}_{\tilde{x} \sim \mathcal{\tilde{X}}} \big[|f^{\theta}_s(\tilde{x})| \big] \geq \epsilon,
% \label{eq:shortcut_feature}
% \end{equation}
% where $s$ is the index of the shortcut feature. $\rho$ and $\epsilon$ are the thresholds indicating high activation for the seen and unseen data distributions. 
% \label{def:shortcut_feature}
% \vspace{-0.1cm}
% \end{definition}

% Note that a shortcut feature, e.g., an animal's legs, can be observed from the unseen instance, because it is not an intrinsic feature.

% \begin{definition}{\sc (Non-shortcut Feature)}.
% Let $x$ and $\tilde{x}$ be the instances from seen and unseen data distributions $\mathcal{X}$ and $\mathcal{\tilde{X}}$, respectively, where $\mathcal{X}\cap\mathcal{\tilde{X}}=\emptyset$. We call a feature a \emph{non-shortcut} if it is highly activated only for the seen instance in expectation. That is,
% \vspace{-0.05cm}
% \begin{equation}
% f^{\theta}_{n}(\rho, \epsilon) : \mathbb{E}_{x \sim \mathcal{X}} \big[|f^{\theta}_n(x)| \big] \geq \rho ~\land ~ \mathbb{E}_{\tilde{x} \sim \mathcal{\tilde{X}}} \big[|f^{\theta}_n(\tilde{x})| \big] < \epsilon. %\qed
% \label{eq:non_shortcut_feature}
% \end{equation}
% \label{def:non_shortcut_feature}
% \vspace{-0.7cm}
% \end{definition}

% \smallskip
% \noindent{\textbf{Property of Shortcut Feature.}} Due to a DNN's simplicity bias, the shortcut features tends to have higher activation values than the non-shortcut features\,\cite{shah2020pitfalls, pezeshki2021gradient}, such that
% \begin{equation}
% \mathbb{E}_{s\in \mathcal{S}} \big[|f^{\theta}_s(x)| \big]> \mathbb{E}_{n\in \mathcal{N}} \big[|f^{\theta}_n(x)| \big],
% \label{eq:shortcut_feature_property}
% \end{equation}
% where $\mathcal{S}$ and $\mathcal{N}$ are the set of the indices of shortcut and non-shortcut features, respectively.

% % ==========================================================================

% \section{Proposed Method: \algname{}}
% \label{sec:methodology}

% \algname{} realizes adaptive feature suppression thorough (a) \emph{attentive debiasing} with \emph{feature map fusion} and (b) \emph{adaptive intensity shifting}. The former drops high-attention features which are expected to be shortcuts, following the guidance from the latter in the form an adjusted drop intensity. Figure \ref{fig:model_arch} illustrates the detailed procedure of \algname{}. While (a) attentive debiasing is executed during the learning process, the drop intensity $\kappa$ is periodically adjusted by (b) adaptive intensity shifting. \algname{} can be implemented on top of any replay-based OCL methods, and see the implementation detail in Appendix A.


% \subsection{Attentive Debiasing}
% \label{subsec: Attentive Debiasing Layer}

% The shortcut features generally exhibit higher attention scores than the non-shortcut feature by Eq.\ \eqref{eq:shortcut_feature_property}. In addition, this shortcut bias usually appears as local or background cues\,\cite{scimeca2021shortcut}. Thus, after fusing the feature maps of different levels, we generate a \textrm{drop mask} to debias the effect of local or background cues on the feature activation.

% \smallskip
% \noindent{\textbf{Feature Map Fusion.}}
% The high-level features are essential to obtain discriminative signals, but they lack fine-grained details\,\cite{zhong2019shallow,wei2021shallow}, e.g., boundaries of objects. The low-level features embrace structural information with more details, which is helpful for accurately finding shortcut regions. Thus, feature map fusion is conducted to reduce the ambiguity in identifying the shortcut regions. Specifically, as shown in Figure \ref{fig:model_arch}(a), given a small memory footprint, we fuse the feature maps ${F}_{first}\in\mathbb{R}^{h\times w\times c}$ and ${F}_{last}$ $\in\mathbb{R}^{h^{\prime}\times w^{\prime}\times c^{\prime}}$ respectively from the first and last layers. To fuse the feature maps with different resolutions, i.e., $\langle {h, w, c}\rangle \neq \langle {h^{\prime}, w^{\prime}, c^{\prime} }\rangle$, the last layer's feature map $F_{last}$ is up-sampled to have the same resolution as the first layer's feature map $F_{first}$ such that $h^{\prime}=h$ and $w^{\prime}=w$. Then, we conduct average pooling along the channel dimension, compressing the outputs of all $c$ channels to produce the attention map ${A}_{fuse}$, which is formulated as
% \begin{equation}
% \begin{gathered}
% {F}_{fuse} = {F}_{first}\odot {\rm Upsample}({F}_{last})\in\mathbb{R}^{h\times w \times c}~~\text{and}\\
% {A}_{fuse} = {\rm ChannelPool}(F_{fuse})\in\mathbb{R}^{h\times w},
% \end{gathered}
% \label{eq:feature_fusion}
% \end{equation}
% where {\rm ChannelPool($\cdot$)} is the pooling along the channel, and $\odot$ is the element-wise tensor product.

% \smallskip
% \noindent{\textbf{Drop Mask Generation.}} 
% Given a drop intensity $\kappa\%$ for each class\footnote{The class is used only during the training process for debiasing. We do not perform such feature suppression in the middle of testing.}, we generate a \textit{drop mask} $M \in \mathbb{R}^{h \times w}$ based on the attention map ${A}_{fuse}$ in Eq.\ \eqref{eq:feature_fusion}. The mask at $(i,j)$ in $M$ is determined by
% \begin{equation}
% M_{i,j} =
% \begin{cases}
% 0 & \text{if}\!\!\quad (i,j) \in {\rm top\text{-}}\kappa(A_{fuse}) \\ 
% 1 & \text{otherwise},\\ 
% \end{cases}
% \label{eq:drop_mask}
% \end{equation}
% where ${\rm top\text{-}}\kappa(A_{fuse})$ returns the set of the top-$\kappa\%$ elements of $A_{fuse}$.
% %
% Last, we apply the drop mask to the first feature map ${F}_{first}$ after the stem layer of a backbone convolutional neural network\,(CNN), e.g., the feature map obtained by the first convolutional stem layer in ResNet18,
% \begin{equation}
% \Tilde{F}_{first} = M \odot {F}_{first}.
% \label{eq:drop_ops}
% \end{equation}
% This masking process affects all succeeding layers along the forward process. The masked feature map $\Tilde{F}_{first}$ accomplishes debiasing by using only the attention scores which can be computed on the fly.


% \subsection{Adaptive Intensity Shifting}
% \label{subsec: Adaptive Debiasing Intensity Scheduler}

% The extent of the shortcut bias naturally varies depending on the incoming tasks and the learning progress of a DNN model. Thus, \textit{adaptive intensity shifting} aims to guide {attentive debiasing} by adaptively adjusting the drop intensity $\kappa$ in a timely manner. The drop intensity is maintained separately for each class. It is \emph{decreased} if the removal of features is expected to lose important non-shortcut features which have high predictive power, \emph{increased} if the removal of features is expected to help emphasize important non-shortcut features, and \emph{unchanged} in neither of the cases,
% \begin{equation}
% \kappa \leftarrow \begin{cases}
% \kappa^\prime * \alpha & \text{if decrement} \\
% \kappa^\prime * (1/\alpha) & \text{if increment} \\
% \kappa^\prime & \text{otherwise},
% \end{cases}
% \label{eq:shifting}
% \end{equation}
% where $\kappa^\prime$ is the preceding value, and $\alpha$\,$(<1.0)$ is a hyperparameter that indicates the shift step.

% \smallskip
% \noindent{\textbf{Loss Collection.}} 
% To classify each case, we focus on the contribution to the reduction of the training loss because a better choice of the drop intensity leads to a better training performance\,\cite{scimeca2021shortcut, geirhos2020shortcut}. To determine whether a decrement or an increment is preferable, two potential values $\kappa=\kappa^\prime * \alpha$ and $\kappa=\kappa^\prime * (1/\alpha)$ alternate every $p$ iterations. The loss reductions are computed at the end of every $p$ iterations and maintained in the set $\mathcal{H}^{dec}$ when $\kappa^\prime * \alpha$ is used and in the set $\mathcal{H}^{inc}$ when $\kappa^\prime * (1/\alpha)$ is used, as shown in Figure \ref{fig:model_arch}(b),
% \begin{equation}
% \begin{gathered}
% \tiny
% \,\,\,{\mathcal{H}}^{dec} = \{\Delta\mathcal{L}_0,\Delta\mathcal{L}_{2p},\dots,\Delta\mathcal{L}_{2p(l-1)}\} \text{\small and} \\
% {\mathcal{H}}^{inc} = \{\underbrace{\Delta\mathcal{L}_{p},\Delta\mathcal{L}_{3p},\dots,\Delta\mathcal{L}_{2pl}}_{\text{Collect  } \Delta\mathcal{L} \text{  every  } 2p \text{  iterations}}\},
% \end{gathered}
% \end{equation}
% where $\Delta\mathcal{L}_{(q+1)\cdot p} = \mathcal{L}_{q\cdot p}-\mathcal{L}_{(q+1)\cdot p}$, and $\mathcal{L}_{(q+1) \cdot p}$ is the expected cross-entropy loss on the samples of a specific class in the memory buffer using the model at the iteration $(q+1)\cdot p$. Note that we compute the loss using the samples in the memory buffer rather than in a batch to obtain a more generalizable training loss. Those loss reductions are recorded until ${\mathcal{H}}^{dec}$ and ${\mathcal{H}}^{inc}$ have $l$ elements. Only a single model is needed to compare two shift directions, preserving the memory constraint of OCL.

% \smallskip
% \noindent{\textbf{Statistical Test and Update.}}
% When ${\mathcal{H}}^{dec}$ and ${\mathcal{H}}^{inc}$ become full every $2\cdot p \cdot l$ iterations, we conduct $t$-test to evaluate if one direction is statistically significant than the other with respect to the loss reduction, i.e., either $p$-value $\leq 0.05$ or $p$-value $\geq 0.95$. If a better direction exists, the preceding value is updated to the better direction; otherwise, it remains the same. Algorithm \ref{alg:pseudocode_adaptive_scheduler} describes the pseudocode of adaptive intensity shifting, which is self-explanatory.

% \input{figures/algorithm_adaptive_scheduler}

% \smallskip
% \noindent{\textbf{Training Data Stabilization.}}
% Furthermore, we consider the side effect of shifting the drop intensity during training. If it changes over time, the distribution of input features could be swayed inconsistently. As widely claimed in \cite{ioffe2015batch, zhou2022online}, this problem often causes training instability and eventually deteriorates the overall performance. In this sense, we decide to drop $\gamma\%$ of the features \emph{constantly}. Thus, $\kappa$ cannot grow beyond $\gamma$; if $\kappa < \gamma$, $(\gamma-\kappa)$\% of the features are additionally chosen uniformly at random among those whose drop mask is not $1$.


% \subsection{Understanding of Shortcut Bias in OCL}
% \label{sec:theoretical_analysis}

% From a theoretical standpoint, we clarify two detrimental effects of learning shortcut features in OCL. See Appendix B for relevant empirical evidences. Let $g^{\text{w}}_i:\mathbb{R}\rightarrow\mathbb{R}^{k}$ be the multiplication of an $i$-th column vector of the weight matrix $\text{w}$ and an $i$-th feature $f_i^\theta$. Then, $g^{\text{w}}_i(f^{\theta}_i(x))$ denotes the contribution of the $i$-th feature to a prediction, i.e., how much the $i$-th feature $f^{\theta}_i(x)$ contributes to the prediction $g^{\text{w}}(f^{\theta}(x))$, since $g^{\text{w}}(f^{\theta}(x))= \sum_{i=1}^d{g^{\text{w}}_i(f^{\theta}_i(x))}$. Here, we formulate low transferability and high forgetability of shortcut features in OCL.

% \begin{property}[{\sc Low Transferability}]
% A shortcut feature of the current task hinders the model from learning the knowledge of the next task.
% \end{property}
% \begin{proof}
% Let's consider training a classifier for the ($t$+1)-th task, given a shortcut biased model $\theta_t$ as the initial model. By Eq.~\eqref{eq:shortcut_feature}, $\mathbb{E}_{x_{t+1} \sim \mathcal{X}_{t+1}}\big[|f^{\theta_t}_s(x_{t+1})| \big] \geq \epsilon$ if $x_{t+1}$ shares the same shortcut features with $x_t$. Then, when training a new model $\theta_{t+1}$ from the model $\theta_{t}$, the shortcut feature $f^{\theta_t}_s$ is no longer discriminative since it can appear in both $\mathcal{X}_{t}$ and $\mathcal{X}_{t+1}$. Thus, the model $\theta_{t+1}$ should learn a totally new discriminative feature, meaning that the model $\theta_{t+1}$  starts from a poor initialization. As a result, the training convergence becomes slower compared with a non-biased model $\theta_t^*$.
% \end{proof}

% \begin{property}[{\sc High Forgetability}]
% A shortcut feature of the current task makes the model forget the knowledge of the previous tasks.
% \end{property}
% \begin{proof}
% Given the previous tasks at $t^{\prime}\in\{1,\ldots,t-1\}$ and the current task at $t$, let's assume that we trained a shortcut biased classifier $\theta_t$.
% Then, the shortcut feature $s$ of $f^{\theta_t}$ contributes to predict the class $y_t\in\mathcal{Y}_t$ such that $\argmax g^{\text{w}_t}_s(f^{\theta_t}_s(x_t))=y_t\in\mathcal{Y}_t$. However, by Eq.~\eqref{eq:shortcut_feature}, $\mathbb{E}_{x_{t^{\prime}} \sim \mathcal{X}_{t^{\prime}}}\big[|f^{\theta_t}_s(x_{t^{\prime}})| \big] \geq \epsilon$ if $x_{t^{\prime}}$ shares the same shortcut features with $x_{t}$.
% Then, even for the previous instance $x_{t^{\prime}}$, the shortcut feature $s$ contributes to predict the class $y_{t}\in\mathcal{Y}_{t}$ such that $\argmax g^{\text{w}_t}_s(f^{\theta_t}_s(x_{t^{\prime}}))=y_t\notin\mathcal{Y}_{t^{\prime}}$, which is a wrong prediction.
% Due to the high activation of shortcut features in Eq.~\eqref{eq:shortcut_feature_property}, this wrong feature contribution gives a significant impact to the final prediction $g^{\text{w}}(f^{\theta}(x_{t^{\prime}}))= \sum_{i=1}^d{g^{\text{w}}_i(f^{\theta}_i(x_{t^{\prime}}))}$, so that the model highly forgets the knowledge of the previous tasks. 
% \end{proof}




% % \subsection{Empirical Proofs of Two Properties}
% % \label{sec:empirical_shorcut_bias_ocl}

% % \begin{figure}[!t]
% %     \centering
% %     \includegraphics[width=0.9\columnwidth]{figures/preliminary_two.pdf}
% %     \hspace{2cm} \small (a) Transferability. \hspace{1.5cm} (b) Forgetability
% %     \vspace{-0.1cm}
% %     \caption{(a) shows lower transferability and (b) shows higher forgetting of shortcut features compared to non-shortcut features.
% %     %(a) shows low transferability in learning task 2 of B-MNIST\,(green 2 and 3) and (b) represents strong forgetting in task 1 after learning task 2 of B-MNIST\,(red 2 and green 3).
% % }
% %     \label{fig:preliminary_exp}
% % \end{figure}

% % %\subsection{Shortcut Induced Performance Degradation}
% % %\label{subsec:preliminary-exp}

% % %\smallskip\smallskip\noindent{\textbf{Experiment setup.}} 
% % To empricially investigate the aforementioned two properties, we conduct a simple controlled experiment using two datasets; MNIST\,\cite{lecun1998gradient} and Biased MNIST (B-MNIST)\,\cite{bahng2020learning}, which is widely utilized in bias learning~\cite{bahng2020learning,bui2021exploiting,tartaglione2021end}.
% % In B-MNIST, each digit is on a different colored background; 0 on red and 1 on green.
% % DNNs trained on B-MNIST employ only color shortcut features for classification because color is a simpler feature than shape of digits.
% % We train ER\,\cite{rolnick2019experience} for OCL setup with two tasks--- Task 1 (T1): classify 0 and 1, and Task 2 (T2): classify 2 and 3.
% % % How to expose color bias on B-MNIST?

% % \smallskip\noindent{\textbf{Low Transferability.}}
% % To validate the transferability, we designate the background color for T2 of B-MNIST as green for both digits 2 and 3.
% % Figure \ref{fig:preliminary_exp}(a) shows the lower transferability of shortcut features than that of non-shortcut features.
% % When training T2, ER trained on B-MNIST (the shortcut biased model) shows slower increase of test accuracy than ER trained on MNIST, since red and green color features learned in T1 are not helpful to generalize well in T2.
% % This indicates that the transferability of the OCL model significantly deteriorates once the model is biased to the shortcut features.

% % \smallskip\noindent{\textbf{High Foregetability.}}
% % To validate the forgetability, we designate the background color for T2 of B-MNIST as green for digit 2 and red for digit 3.
% % Figure \ref{fig:preliminary_exp}(b) shows the higher forgetability of shortcut features than that of non-shortcut features.
% % After training task 2, ER trained on B-MNIST shows rapid forgetting of the class prediction in T1, since the red or green color becomes a shortcut cue to predict the digit 2 or 3 in T2.
% % This indicates that the OCL model also be significantly threatened by forgetting once the model is biased to the shortcut features.


% \begin{comment}
% The empirical results in Figure \ref{fig:preliminary_exp} support the underlying claim that the adverse effect of shortcut learning to transferability and forgetting. The experiments were conducted on sequential Biased MNIST\,(B-MNIST)\,\cite{bahng2020learning} where different colors are designated for each digit as shortcut. 
% The accuracy of a widely applied OCL method, ER\,\cite{rolnick2019experience}, trained on B-MNIST in Figure \ref{fig:preliminary_exp}(a) shows shortcut bias on color while overlooking shape of digits.
% As in Figure \ref{fig:preliminary_exp}(b), stronger forgetting is observed in the model biased on shortcut when the color feature is no longer discriminative for classifying the first task. The model with color bias also suffers from lower transferability and we speculate that the color bias does not generalize well to unseen new classes, as in Figure \ref{fig:preliminary_exp}(c).
% % learns the semantically dissimilar task\,(e.g., classifying two same color digits) requiring a feature\,(e.g., shape) other than color, as in Figure \ref{fig:preliminary_exp}(c).
% \end{comment}
